The Topological form is the Pfaffian form

For a given graph $G$, Budzik, Gaiotto, Kulp, Wang, Williams, Wu, Yu, and the first author studied a ''topological'' differential form $\alpha_G$, which expresses violations of BRST-closedness of a quantum field theory along a single topological direction. In a seemingly unrelated context, Brown, Panzer, and the second author studied a ''Pfaffian'' differential form $\phi_G$, which is used to construct cohomology classes of the odd commutative graph complex. We give an explicit combinatorial proof that $\alpha_G$ coincides with $\phi_G$. We also discuss the equivalence of several properties of these forms, which had been established independently for both contexts in previous work.

==> tikzlibrarypenrose.code.tex <==
%%
%% This is file `tikzlibrarypenrose.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tilings_code.dtx  (with options: `penrosedep')
%% ----------------------------------------------------------------
%% tilings --- TikZ library for producing tilings
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\ProvidesFile {tikzlibrarypenrose.code.tex}
 [2023/06/01 v2.0 TikZ pics for Penrose tiles]
\usetikzlibrary{tilings.penrose}
\ExplSyntaxOn
\NewDocumentCommand \SetPenrosePath { m }
{
  \__tilings_set_tiling_path:n {#1}
}
\NewDocumentCommand \BakePenroseTile {m}
{
  \__tilings_bake_tile:n {#1}
}
\NewDocumentCommand \MakePenroseTile {m}
{
  \__tilings_bake_tile:n {#1}
}
\NewDocumentCommand \UsePenroseTile {O{} m}
{
  \__tilings_use_tile:nn {#1}{#2}
}
\NewDocumentCommand \PenroseDecomposition { O{} m m m }
{
 \__tilings_tiling_decomposition:nnnn {#1}{#2}{#3}{#4}
}
\ExplSyntaxOff
\tikzset{
  save Penrose path/.forward to=/tikz/save tiling path,
  clone Penrose side path/.forward to=/tikz/clone tiling side path,
  spath/prefix/Penrose side/.forward to=/tikz/spath/prefix/tiling side,
  spath/suffix/Penrose side/.forward to=/tikz/spath/suffix/tiling side,
  clone Penrose tile path/.forward to=/tikz/clone tiling tile path,
  spath/prefix/Penrose tile/.forward to=/tikz/spath/prefix/tiling tile,
  spath/suffix/Penrose tile/.forward to=/tikz/spath/suffix/tiling tile,
  Penrose step/.forward to=/tikz/tiling step,
  every tile/.append style={
    every Penrose tile/.try
  },
  every tile clip/.append style={
    every Penrose tile clip/.try
  },
  every tile pic/.append style={
    every Penrose pic/.try
  },
  tile/.append style={
    Penrose tile #1/.try,
    Penrose tile/.try=#1
  }
}
%% 
%% Copyright (C) 2014-2023 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  penrose_code.dtx
%%                                  penrose.tex
%% and the derived files            penrose.ins
%%                                  penrose_code.pdf
%%                                  penrose.pdf
%%                                  tikzlibrarytilings.code.tex
%%                                  tikzlibrarytilings.penrose.code.tex
%%                                  tikzlibrarytilings.polykite.code.tex
%%                                  tikzlibrarypenrose.code.tex
%%                                  README.txt
%% 
%%
%% End of file `tikzlibrarypenrose.code.tex'.


==> tikzlibrarytilings.code.tex <==
%%
%% This is file `tikzlibrarytilings.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tilings_code.dtx  (with options: `tilings')
%% ----------------------------------------------------------------
%% tilings --- TikZ library for producing tilings
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\ProvidesExplFile
      {tikzlibrarytilings.code.tex}
      {2023/06/01}
      {2.0}
      {TikZ pics for tilings such as Penrose tiles}
\RequirePackage{tikz}
\usetikzlibrary{spath3}
\ExplSyntaxOn
\tl_new:N \g__tilings_side_a_tl
\tl_new:N \g__tilings_side_b_tl
\tl_new:N \g__tilings_side_c_tl
\tl_new:N \g__tilings_side_d_tl
\tl_new:N \g__tilings_side_e_tl
\tl_new:N \g__tilings_side_A_tl
\tl_new:N \g__tilings_side_B_tl
\tl_new:N \g__tilings_side_C_tl
\tl_new:N \g__tilings_side_D_tl
\tl_new:N \g__tilings_side_E_tl
\tl_new:c {g__tilings_side_1_tl}
\tl_new:c {g__tilings_side_2_tl}
\tl_new:c {g__tilings_side_3_tl}
\tl_gset:Nn \g__tilings_side_a_tl
{
  \pgfsyssoftpath@movetotoken{0pt}{0pt}
  \pgfsyssoftpath@linetotoken{1pt}{0pt}
}
\tl_gset_eq:NN \g__tilings_side_b_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_c_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_d_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_e_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_A_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_B_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_C_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_D_tl \g__tilings_side_a_tl
\tl_gset_eq:NN \g__tilings_side_E_tl \g__tilings_side_a_tl
\tl_gset_eq:cN {g__tilings_side_1_tl} \g__tilings_side_a_tl
\tl_gset_eq:cN {g__tilings_side_2_tl} \g__tilings_side_a_tl
\tl_gset_eq:cN {g__tilings_side_3_tl} \g__tilings_side_a_tl
\fp_new:N \l__tilings_tmpa_fp
\fp_new:N \l__tilings_tmpb_fp
\fp_new:N \l__tilings_tmpc_fp
\fp_new:N \l__tilings_saved_x_fp
\fp_new:N \l__tilings_saved_y_fp
\str_new:N \l__tilings_tmpa_str
\str_new:N \l__tilings_tmpb_str
\seq_new:N \l__tilings_tmpa_seq
\tl_new:N \l__tilings_tmpa_tl
\tl_new:N \l__tilings_tmpb_tl
\tl_new:N \l__tilings_tmpc_tl
\tl_new:N \l__tilings_tmpd_tl
\tl_new:N \l__tilings_tmp_tile_path_tl
\tl_new:N \l__tilings_action_lms_tl
\tl_new:N \l__tilings_parameters_lms_tl
\int_new:N \l__tilings_tmpa_int
\int_new:N \l__tilings_tmpb_int
\fp_new:N \l__tilings_xa_fp
\fp_new:N \l__tilings_ya_fp
\fp_new:N \l__tilings_xb_fp
\fp_new:N \l__tilings_yb_fp
\dim_new:N \l__tilings_xa_dim
\dim_new:N \l__tilings_ya_dim
\dim_new:N \l__tilings_xb_dim
\dim_new:N \l__tilings_yb_dim
\dim_new:N \g__tilings_xa_dim
\dim_new:N \g__tilings_ya_dim
\dim_new:N \g__tilings_xb_dim
\dim_new:N \g__tilings_yb_dim
\prop_new:N \l__tilings_tmpa_prop
\bool_new:N \l__tilings_cw_bool
\bool_new:N \l__tilings_update_saved_bool
\bool_new:N \l__tilings_relative_bool
\bool_new:N \l__tilings_edge_bool
\str_const:Nn \c__tilings_colon_str {:}
\str_const:Nn \c__tilings_comma_str {,}
\fp_const:Nn \c__tilings_cm_fp {\dim_to_fp:n {1cm}}
\tl_new:N \g__tilings_output_tl
\fp_new:N \g__tilings_output_a_fp
\fp_new:N \g__tilings_output_b_fp
\prop_new:N \g__tilings_tilenames_prop
\regex_const:Nn \c__tilings_anchor_regex {\s\w+\Z}
\cs_generate_variant:Nn \seq_set_split:Nnn {NVV}
\cs_generate_variant:Nn \regex_extract_once:NnNTF {NVNTF}
\cs_generate_variant:Nn \tl_if_eq:nnT {nVT}
\cs_generate_variant:Nn \tl_if_in:NnT {NVT}
\cs_generate_variant:Nn \prop_item:Nn {cV}
\cs_generate_variant:Nn \tl_if_head_is_group_p:n {V}
\msg_new:nnn { tilings }{ not baked }
{ Tile~ #1~ has~ not~ been~ baked. }
\msg_new:nnn { tilings }{ no tile }
{ Tile~ #1~ has~ not~ been~ defined. }
\msg_new:nnn { tilings }{ no side }
{ Tile~ side~ #1~ has~ not~ been~ defined,~ using~ default. }
\msg_new:nnn { tilings }{ tile no edge }
{ Tile~ #1~ doesn't~ have~ an~ edge~ labelled~ #2;
  ~ available~ edges~ are~ #3.}
\msg_new:nnn { tilings }{ no edge }
{ Either~ tile~ #1~ doesn't~ exist
  ~ or~ it~ doesn't~ have~ an~ edge~ labelled~ #2.}
\cs_new_nopar:Npn \__tilings_normalise_path:Nn #1#2
{
  \group_begin:
  \spath_initialpoint:Nn \l__tilings_tmpa_tl {#2}
  \fp_set:Nn \l__tilings_tmpa_fp {\tl_head:N \l__tilings_tmpa_tl}
  \tl_set:Nx \l__tilings_tmpa_tl {\tl_tail:N \l__tilings_tmpa_tl}
  \fp_set:Nn \l__tilings_tmpb_fp {\tl_head:N \l__tilings_tmpa_tl}
  \spath_finalpoint:Nn \l__tilings_tmpa_tl {#2}
  \fp_set:Nn \l__tilings_tmpa_fp
  {\tl_head:N \l__tilings_tmpa_tl - \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpa_tl {\tl_tail:N \l__tilings_tmpa_tl}
  \fp_set:Nn \l__tilings_tmpb_fp
  {\tl_head:N \l__tilings_tmpa_tl - \l__tilings_tmpb_fp}
  \fp_set:Nn \l__tilings_tmpc_fp
  {\l__tilings_tmpa_fp^2 + \l__tilings_tmpb_fp^2}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_tmpa_fp/\l__tilings_tmpc_fp}
  \fp_set:Nn \l__tilings_tmpb_fp {\l__tilings_tmpb_fp/\l__tilings_tmpc_fp}
  \fp_set:Nn \l__tilings_tmpc_fp {-\l__tilings_tmpb_fp}
  \tl_set:Nx \l__tilings_tmpb_tl
  {
    {\fp_use:N \l__tilings_tmpa_fp}
    {\fp_use:N \l__tilings_tmpc_fp} % swapped
    {\fp_use:N \l__tilings_tmpb_fp} % swapped
    {\fp_use:N \l__tilings_tmpa_fp}
  }
  \spath_initialpoint:Nn \l__tilings_tmpa_tl {#2}
  \fp_set:Nn \l__tilings_tmpa_fp
  {
    (-1) * \l__tilings_tmpa_fp * \tl_head:N \l__tilings_tmpa_tl
    + (-1) * \l__tilings_tmpb_fp * \tl_tail:N \l__tilings_tmpa_tl
  }
  \fp_set:Nn \l__tilings_tmpb_fp
  {
    (-1) * \l__tilings_tmpa_fp * \tl_tail:N \l__tilings_tmpa_tl
    +  \l__tilings_tmpb_fp * \tl_head:N \l__tilings_tmpa_tl
  }
  \tl_put_right:Nx \l__tilings_tmpb_tl {
    {\fp_to_dim:N \l__tilings_tmpa_fp}
    {\fp_to_dim:N \l__tilings_tmpb_fp}
  }
  \spath_transform:NnV \l__tilings_tmpa_tl {#2} \l__tilings_tmpb_tl
  \tl_gset_eq:NN \g__tilings_output_tl \l__tilings_tmpa_tl
  \group_end:
  \tl_set_eq:NN #1 \g__tilings_output_tl
  \tl_gclear:N \g__tilings_output_tl
}
\cs_generate_variant:Nn \__tilings_normalise_path:Nn {NV, cn, cV}
\cs_new_protected_nopar:Npn \__tilings_normalise_path:N #1
{
  \__tilings_normalise_path:NV #1#1
}
\cs_generate_variant:Nn \__tilings_normalise_path:N {c}
\cs_new_protected_nopar:Npn \__tilings_set_tiling_path:n #1
{
  \group_begin:
  \pgfsyssoftpath@getcurrentpath\l__tilings_tmpa_tl
  \__tilings_normalise_path:N \l__tilings_tmpa_tl
  \tl_gset_eq:cN {g__tilings_side_#1_tl} \l__tilings_tmpa_tl
  \group_end:
}

\NewDocumentCommand \SetTilingPath { m }
{
  \__tilings_set_tiling_path:n {#1}
}
\cs_new_nopar:Npn \tikz_scan_point:n #1
{
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
}
\cs_generate_variant:Nn \tikz_scan_point:n {V}
\prg_new_conditional:Npnn \tikz_node_if_defined:n #1 {p,T,F,TF}
{
  \tl_if_exist:cTF {pgf@sh@ns@\use:c{tikz@pp@name}{#1}}
  {
    \prg_return_true:
  }{
    \tl_if_exist:cTF
    {pgf@sh@ns@not yet positionedPGFINTERNAL\use:c{tikz@pp@name}{#1}}
    {
      \pgf_return_true:
    }
    {
      \prg_return_false:
    }
  }
}
\cs_new_nopar:Npn \__tilings_keys_get:Nn #1#2
{
  \pgfkeysgetvalue{/tikz/tiling/#2}{#1}
}
\cs_new_nopar:Npn \__tilings_keys_get:n #1
{
  \pgfkeysvalueof{/tikz/tiling/#1}
}
\cs_new_nopar:Npn \__tilings_tikz_keys_get:Nn #1#2
{
  \pgfkeysgetvalue{/tikz/#2}{#1}
}
\cs_new_nopar:Npn \__tilings_tikz_keys_get:n #1
{
  \pgfkeysvalueof{/tikz/#1}
}
\cs_new_nopar:Npn \__tilings_pgf_keys_get:Nn #1#2
{
  \pgfkeysgetvalue{#2}{#1}
}
\cs_new_nopar:Npn \__tilings_pgf_keys_get:n #1
{
  \pgfkeysvalueof{#1}
}
\cs_new_nopar:Npn \__tilings_make_tile:nnn #1#2#3
{
  \group_begin:
  \tl_set:Nn \l__tilings_tmpa_tl {#3}
  \tl_set:Nx \l__tilings_tmpb_tl {\tl_head:N \l__tilings_tmpa_tl}
  \tl_set:Nn \l__tilings_tmpa_tl {\pgfsyssoftpath@movetotoken}
  \tl_put_right:Nx \l__tilings_tmpa_tl
  {
    {
      \fp_to_dim:n
      {(\tl_item:Nn \l__tilings_tmpb_tl {1}) * \c__tilings_cm_fp}
    }
    {
      \fp_to_dim:n
      {(\tl_item:Nn \l__tilings_tmpb_tl {2}) * \c__tilings_cm_fp}
    }
  }
  \tl_set_eq:NN \l__tilings_tmp_tile_path_tl \l__tilings_tmpa_tl
  \tl_set:Nn \l__tilings_tmpa_tl {#3}
  \tl_put_right:Nx \l__tilings_tmpa_tl {{\tl_head:N \l__tilings_tmpa_tl}}
  \tl_map_inline:nn {#2} {
    \tl_set:Nx \l__tilings_tmpc_tl {\tl_head:n {##1}}
    \tl_if_exist:cF {g__tilings_side_ \tl_use:N \l__tilings_tmpc_tl _tl}
    {
      \msg_error:nnx { tilings }{ no side } { \tl_use:N \l__tilings_tmpc_tl }
      \tl_gset_eq:cc
      {g__tilings_side_ \tl_use:N \l__tilings_tmpc_tl _tl}
      {g__tilings_side_a_tl}
    }
    \tl_set_eq:Nc \l__tilings_tmpd_tl
    {g__tilings_side_ \tl_use:N \l__tilings_tmpc_tl _tl}
    \tl_set:Nx \l__tilings_tmpb_tl {\tl_head:N \l__tilings_tmpa_tl}
    \tl_set:Nx \l__tilings_tmpa_tl {\tl_tail:N \l__tilings_tmpa_tl}
    \fp_set:Nn \l__tilings_tmpa_fp
    { \tl_item:Nn \l__tilings_tmpb_tl {1} }
    \fp_set:Nn \l__tilings_tmpb_fp
    { \tl_item:Nn \l__tilings_tmpb_tl {2} }
    \tl_set:Nx \l__tilings_tmpb_tl {\tl_head:N \l__tilings_tmpa_tl}
    \fp_set:Nn \l__tilings_tmpa_fp
    {\tl_item:Nn \l__tilings_tmpb_tl {1} - \l__tilings_tmpa_fp}
    \fp_set:Nn \l__tilings_tmpb_fp
    {\tl_item:Nn \l__tilings_tmpb_tl {2} - \l__tilings_tmpb_fp}
    \fp_set:Nn \l__tilings_tmpc_fp {-\l__tilings_tmpb_fp}
    \tl_set:Nx \l__tilings_tmpb_tl
    {
      {\fp_to_dim:n { \l__tilings_tmpa_fp * \c__tilings_cm_fp }}
      {\fp_to_dim:n { \l__tilings_tmpb_fp * \c__tilings_cm_fp }}% not swapped
      {\fp_to_dim:n { \l__tilings_tmpc_fp * \c__tilings_cm_fp }}% not swapped
      {\fp_to_dim:n { \l__tilings_tmpa_fp * \c__tilings_cm_fp }}
      {0}
      {0}
    }
    \spath_transform:NV \l__tilings_tmpd_tl \l__tilings_tmpb_tl
    \spath_weld:NV \l__tilings_tmp_tile_path_tl \l__tilings_tmpd_tl
  }
  \spath_close:N \l__tilings_tmp_tile_path_tl
  \tl_gset_eq:NN \g__tilings_output_tl \l__tilings_tmp_tile_path_tl
  \group_end:
  \tl_gclear_new:c {g__tilings_tile_#1_tl}
  \tl_gset_eq:cN {g__tilings_tile_#1_tl} \g__tilings_output_tl
  \tl_gclear:N \g__tilings_output_tl
}
\cs_new_nopar:Npn \__tilings_make_tile:nn #1#2
{
  \__tilings_make_tile:nnn {#1} #2
}
\cs_generate_variant:Nn \__tilings_make_tile:nn {nV}
\prop_new:N \g__tilings_tiles_prop
\cs_new_nopar:Npn \__tilings_add_coordinate:Nnn #1#2#3 {
  \group_begin:
  \fp_set:Nn \l__tilings_tmpa_fp {#2}
  \fp_set:Nn \l__tilings_tmpb_fp {#3}
  \bool_if:NT \l__tilings_relative_bool
  {
    \fp_add:Nn \l__tilings_tmpa_fp {\l__tilings_saved_x_fp}
    \fp_add:Nn \l__tilings_tmpb_fp {\l__tilings_saved_y_fp}
  }
  \fp_gset_eq:NN \g__tilings_output_a_fp \l__tilings_tmpa_fp
  \fp_gset_eq:NN \g__tilings_output_b_fp \l__tilings_tmpb_fp
  \group_end:
  \tl_put_right:Nx #1
  {
    {{\fp_use:N \g__tilings_output_a_fp}{\fp_use:N \g__tilings_output_b_fp}}
  }
  \bool_if:NT \l__tilings_update_saved_bool
  {
    \fp_set_eq:NN \l__tilings_saved_x_fp \g__tilings_output_a_fp
    \fp_set_eq:NN \l__tilings_saved_y_fp \g__tilings_output_b_fp
  }
  \fp_gzero:N \g__tilings_output_a_fp
  \fp_gzero:N \g__tilings_output_b_fp
}
\cs_new_nopar:Npn \__tilings_add_xy_coordinate:w #1#2,#3 \q_stop
{
  \__tilings_add_coordinate:Nnn #1 {#2}{#3}
}
\cs_new_nopar:Npn \__tilings_add_rth_coordinate:w #1#2:#3 \q_stop
{
  \__tilings_add_coordinate:Nnn #1 {(#3) * cosd(#2)}{(#3) * sind(#2)}
}
\cs_new_nopar:Npn \__tilings_transform_side_to_axis:Nnn #1#2#3
{
  \group_begin:
  \prop_get:NnNTF \g__tilings_tiles_prop {#2} \l__tilings_tmpa_tl
  {
  \int_zero:N \l__tilings_tmpb_int
  \int_incr:N \l__tilings_tmpb_int
  \tl_set:Nx \l__tilings_tmpc_tl {\tl_head:N \l__tilings_tmpa_tl}
    \bool_set_false:N \l__tilings_edge_bool
    \tl_map_inline:Nn \l__tilings_tmpc_tl {
      \str_if_eq:nnT {##1} {#3} {
        \bool_set_true:N \l__tilings_edge_bool
        \tl_map_break:
      }
      \int_incr:N \l__tilings_tmpb_int
    }
    \bool_if:NTF \l__tilings_edge_bool
    {
      \tl_set:Nx \l__tilings_tmpc_tl {\tl_tail:N \l__tilings_tmpa_tl}
      \tl_set:Nx \l__tilings_tmpc_tl {\tl_item:Nn \l__tilings_tmpc_tl {1}}
      \tl_put_right:Nx \l__tilings_tmpc_tl
      {{\tl_item:Nn \l__tilings_tmpc_tl {1}}}
      \tl_set:Nx \l__tilings_tmpa_tl
      {\tl_item:Nn \l__tilings_tmpc_tl {\int_use:N \l__tilings_tmpb_int}}
      \tl_set:Nx \l__tilings_tmpb_tl
      {\tl_item:Nn \l__tilings_tmpc_tl {\int_use:N \l__tilings_tmpb_int + 1}}
      \bool_if:NT #1
      {
        \tl_set:NV \l__tilings_tmpc_tl \l__tilings_tmpa_tl
        \tl_set:NV \l__tilings_tmpa_tl \l__tilings_tmpb_tl
        \tl_set:NV \l__tilings_tmpb_tl \l__tilings_tmpc_tl
      }
      \fp_set:Nn \l__tilings_xa_fp {\tl_item:Nn \l__tilings_tmpb_tl {1}}
      \fp_set:Nn \l__tilings_ya_fp {\tl_item:Nn \l__tilings_tmpb_tl {2}}
      \fp_set:Nn \l__tilings_xb_fp
      {\tl_item:Nn \l__tilings_tmpa_tl {1} - \l__tilings_xa_fp}
      \fp_set:Nn \l__tilings_yb_fp
      {\tl_item:Nn \l__tilings_tmpa_tl {2} - \l__tilings_ya_fp}
      \fp_set:Nn \l__tilings_tmpa_fp
      {(\l__tilings_xb_fp)^2 + (\l__tilings_yb_fp)^2}
      \fp_set:Nn \l__tilings_xb_fp { \l__tilings_xb_fp / \l__tilings_tmpa_fp}
      \fp_set:Nn \l__tilings_yb_fp { \l__tilings_yb_fp / \l__tilings_tmpa_fp}
      \tl_gset:Nx \g__tilings_output_tl
      {
        \exp_not:N \pgftransformtriangle
        {
          \exp_not:N \pgfpoint{0pt}{0pt}
        }
        {
          \exp_not:N \pgfpoint
          {\fp_to_dim:N \l__tilings_xb_fp}{\fp_to_dim:n {-\l__tilings_yb_fp}}
        }
        {
          \exp_not:N \pgfpoint
          {\fp_to_dim:N \l__tilings_yb_fp}{\fp_to_dim:N \l__tilings_xb_fp}
        }
        \exp_not:N \pgftransformshift
        {
          \exp_not:N \pgfpoint
          {
            \fp_to_dim:n {-\l__tilings_xa_fp * \c__tilings_cm_fp}
          }
          {
            \fp_to_dim:n {-\l__tilings_ya_fp * \c__tilings_cm_fp}
          }
        }
      }
    }
    {
      \msg_error:nnxxx {tilings} {tile no edge} {#2} {#3}
      {\tl_use:N  \l__tilings_tmpc_tl }
      \tl_gclear:N \g__tilings_output_tl
    }
  }
  {
    \msg_error:nnn {tilings} {no tile} {#2}
    \tl_gclear:N \g__tilings_output_tl
  }
  \group_end:
  \tl_use:N \g__tilings_output_tl
  \tl_gclear:N \g__tilings_output_tl
}
\cs_generate_variant:Nn
\__tilings_transform_side_to_axis:Nnn {Nnx,NnV,NVV}
\cs_new_nopar:Npn \__tilings_translate_vertex_to_origin:Nnn #1#2#3
{
  \group_begin:
  \prop_get:NnNTF \g__tilings_tiles_prop {#2} \l__tilings_tmpa_tl
  {
  \int_zero:N \l__tilings_tmpb_int
  \int_incr:N \l__tilings_tmpb_int
  \tl_set:Nx \l__tilings_tmpc_tl {\tl_head:N \l__tilings_tmpa_tl}
    \bool_set_false:N \l__tilings_edge_bool
    \tl_map_inline:Nn \l__tilings_tmpc_tl {
      \str_if_eq:nnT {##1} {#3} {
        \bool_set_true:N \l__tilings_edge_bool
        \tl_map_break:
      }
      \int_incr:N \l__tilings_tmpb_int
    }
    \bool_if:NTF \l__tilings_edge_bool
    {
      \tl_set:Nx \l__tilings_tmpc_tl {\tl_tail:N \l__tilings_tmpa_tl}
      \tl_set:Nx \l__tilings_tmpc_tl {\tl_item:Nn \l__tilings_tmpc_tl {1}}
      \tl_put_right:Nx \l__tilings_tmpc_tl
      {{\tl_item:Nn \l__tilings_tmpc_tl {1}}}
      \tl_set:Nx \l__tilings_tmpa_tl
      {\tl_item:Nn \l__tilings_tmpc_tl {\int_use:N \l__tilings_tmpb_int}}
      \tl_set:Nx \l__tilings_tmpb_tl
      {\tl_item:Nn \l__tilings_tmpc_tl {\int_use:N \l__tilings_tmpb_int + 1}}
      \bool_if:NT #1
      {
        \tl_set:NV \l__tilings_tmpc_tl \l__tilings_tmpa_tl
        \tl_set:NV \l__tilings_tmpa_tl \l__tilings_tmpb_tl
        \tl_set:NV \l__tilings_tmpb_tl \l__tilings_tmpc_tl
      }
      \fp_set:Nn \l__tilings_xa_fp {\tl_item:Nn \l__tilings_tmpb_tl {1}}
      \fp_set:Nn \l__tilings_ya_fp {\tl_item:Nn \l__tilings_tmpb_tl {2}}
      \tl_gset:Nx \g__tilings_output_tl
      {
        \exp_not:N \pgftransformshift
        {
          \exp_not:N \pgfpoint
          {
            \fp_to_dim:n {-\l__tilings_xa_fp * \c__tilings_cm_fp}
          }
          {
            \fp_to_dim:n {-\l__tilings_ya_fp * \c__tilings_cm_fp}
          }
        }
      }
    }
    {
      \msg_error:nnxxx {tilings} {tile no edge} {#2} {#3}
      {\tl_use:N  \l__tilings_tmpc_tl }
      \tl_gclear:N \g__tilings_output_tl
    }
  }
  {
    \msg_error:nnn {tilings} {no tile} {#2}
    \tl_gclear:N \g__tilings_output_tl
  }
  \group_end:
  \tl_use:N \g__tilings_output_tl
  \tl_gclear:N \g__tilings_output_tl
}
\cs_generate_variant:Nn
\__tilings_translate_vertex_to_origin:Nnn {Nnx,NnV,NVV}
\DeclareDocumentCommand \TransformAlongSide {s m m}
{
  \IfBooleanTF {#1}
  {
    \bool_set_true:N \l__tilings_cw_bool
  }
  {
    \bool_set_false:N \l__tilings_cw_bool
  }
  \__tilings_transform_side_to_axis:Nnx \l__tilings_cw_bool {#2}{#3}
}
\cs_new_nopar:Npn \__tilings_coordinates_at_vertices:n #1
{
  \group_begin:
  \prop_get:NnN \g__tilings_tiles_prop {#1} \l__tilings_tmpa_tl
  \tl_set:Nx \l__tilings_tmpb_tl {\tl_head:N \l__tilings_tmpa_tl}
  \tl_set:Nx \l__tilings_tmpc_tl {\tl_tail:N \l__tilings_tmpa_tl}
  \tl_set:Nx \l__tilings_tmpc_tl
  {\tl_item:Nn \l__tilings_tmpc_tl {1}}
  \tl_put_right:Nx \l__tilings_tmpc_tl
  {{\tl_item:Nn \l__tilings_tmpc_tl {1}}}
  \tl_set:Nx \l__tilings_tmpa_tl {\tl_head:N \l__tilings_tmpc_tl}
  \tl_set:Nx \l__tilings_tmpc_tl {\tl_tail:N \l__tilings_tmpc_tl}
  \tl_map_inline:Nn \l__tilings_tmpb_tl {
    \tl_set:Nx \l__tilings_tmpd_tl {
      \exp_not:N \coordinate
      (-edge~ ##1~ start)~
      at (
      \tl_item:Nn \l__tilings_tmpa_tl {1},
      \tl_item:Nn \l__tilings_tmpa_tl {2}
      );
    }
    \tl_use:N \l__tilings_tmpd_tl
    \tl_set:Nx \l__tilings_tmpa_tl {\tl_head:N \l__tilings_tmpc_tl}
    \tl_set:Nx \l__tilings_tmpc_tl {\tl_tail:N \l__tilings_tmpc_tl}
    \tl_set:Nx \l__tilings_tmpd_tl {
      \exp_not:N \coordinate
      (-edge~ ##1~ end)~
      at (
      \tl_item:Nn \l__tilings_tmpa_tl {1},
      \tl_item:Nn \l__tilings_tmpa_tl {2}
      );
    }
    \tl_use:N \l__tilings_tmpd_tl
  }
  \group_end:
}
\DeclareDocumentCommand \CoordinatesAtVertices {m}
{
  \__tilings_coordinates_at_vertices:n {#1}
}
\tikzset{
  transform~ to~ tile/.code~ args={#1~ along~ #2}{%
    \group_begin:
    \tl_if_in:nnTF {#1} {back}
    {
      \tikzset{
        tiling/alignment~ set~ location=#1,
        tiling/alignment~ direction={backwards}
      }
    }
    {
      \tikzset{
        tiling/alignment~ location=#1,
        tiling/alignment~ direction={forewards}
      }
    }
    \tl_if_in:nnTF {#2} {using}
    {
      \tikzset{
        tiling/alignment~ set~ edges=#2,
      }
    }
    {
      \tikzset{
        tiling/alignment~ edge=#2,
      }
    }
    \tikz_scan_point:n {
      (\__tilings_keys_get:n {alignment~ location}
      -edge~ \__tilings_keys_get:n {alignment~ edge}~ start)
    }
    \dim_set_eq:Nc \l__tilings_xa_dim {pgf@x}
    \dim_set_eq:Nc \l__tilings_ya_dim {pgf@y}
    \tikz_scan_point:n {
      (\__tilings_keys_get:n {alignment~ location}
      -edge~ \__tilings_keys_get:n {alignment~ edge}~ end)
    }
    \dim_set_eq:Nc \l__tilings_xb_dim {pgf@x}
    \dim_set_eq:Nc \l__tilings_yb_dim {pgf@y}
    \__tilings_keys_get:Nn \l__tilings_tmpb_tl {alignment~ direction}
    \tl_if_eq:NnTF \l__tilings_tmpb_tl {forewards}
    {
      \dim_gset_eq:NN \g__tilings_xa_dim \l__tilings_xa_dim
      \dim_gset_eq:NN \g__tilings_ya_dim \l__tilings_ya_dim
      \dim_gset_eq:NN \g__tilings_xb_dim \l__tilings_xb_dim
      \dim_gset_eq:NN \g__tilings_yb_dim \l__tilings_yb_dim
    }
    {
      \dim_gset_eq:NN \g__tilings_xa_dim \l__tilings_xb_dim
      \dim_gset_eq:NN \g__tilings_ya_dim \l__tilings_yb_dim
      \dim_gset_eq:NN \g__tilings_xb_dim \l__tilings_xa_dim
      \dim_gset_eq:NN \g__tilings_yb_dim \l__tilings_ya_dim
    }
    \dim_gsub:Nn \g__tilings_xb_dim {\g__tilings_xa_dim}
    \dim_gsub:Nn \g__tilings_yb_dim {\g__tilings_ya_dim}
    \dim_gset:Nn \g__tilings_xb_dim
    {\g__tilings_xb_dim * \dim_ratio:nn {1pt}{1cm}}
    \dim_gset:Nn \g__tilings_yb_dim
    {\g__tilings_yb_dim * \dim_ratio:nn {1pt}{1cm}}
    \group_end:
    \pgftransformshift{\pgfpoint{\g__tilings_xa_dim}{\g__tilings_ya_dim}}
    \pgftransformtriangle
    {\pgfpoint{0pt}{0pt}}
    {\pgfpoint{\g__tilings_xb_dim}{\g__tilings_yb_dim}}
    {\pgfpoint{-\g__tilings_yb_dim}{\g__tilings_xb_dim}}
  },
  align~ with/.code~ args={#1~ along~ #2}{%
    \tl_if_in:nnTF {#1} {back}
    {
      \tikzset{
        tiling/alignment~ set~ location=#1,
        tiling/alignment~ direction={backwards}
      }
    }
    {
      \tikzset{
        tiling/alignment~ location=#1,
        tiling/alignment~ direction={forewards}
      }
    }
    \tl_if_in:nnTF {#2} {using}
    {
      \tikzset{
        tiling/alignment~ set~ edges=#2,
      }
    }
    {
      \tikzset{
        tiling/alignment~ edge=#2,
      }
    }
    \tikz_node_if_defined:nTF
    {
      \__tilings_keys_get:n {alignment~ location}
      -edge~ \__tilings_keys_get:n {alignment~ edge}~ start
    }
    {
      \tikzset{
        tiling/alignment~ start/.expanded={
          (\__tilings_keys_get:n {alignment~ location}
          -edge~ \__tilings_keys_get:n {alignment~ edge}~ start)
        },
        tiling/alignment~ end/.expanded={
          (\__tilings_keys_get:n {alignment~ location}
          -edge~ \__tilings_keys_get:n {alignment~ edge}~ end)
        },
      }
    }
    {
      \__tilings_keys_get:Nn \l__tilings_tmpa_tl {alignment~ location}
      \tl_set:Nx \l__tilings_tmpa_tl {\tl_use:N \l__tilings_tmpa_tl}
      \prop_get:NVNTF \g__tilings_tilenames_prop
      \l__tilings_tmpa_tl \l__tilings_tmpb_tl
      {
        \prop_get:NVN \g__tilings_tiles_prop
        \l__tilings_tmpb_tl \l__tilings_tmpc_tl
        \msg_error:nnxxx { tilings }{ tile no edge }
        {
          \tl_use:N \l__tilings_tmpa_tl \c_space_tl
          (type~ \tl_use:N \l__tilings_tmpb_tl)
        }
        {\__tilings_keys_get:n {alignment~ edge} }
        { \tl_item:Nn \l__tilings_tmpc_tl {1} }
      }
      {
        \msg_error:nnx { tilings }{ no tile }
        {\__tilings_keys_get:n {alignment~ location} }
      }
    }
  },
  tiling/.is~ family,
  tiling/alignment~ set~ location/.code~ args={#1~ back}{
    \tikzset{
      tiling/alignment~ location=#1,
    }
  },
  tiling/alignment~ set~ edges/.code~ args={#1~ using~ #2}{
    \tikzset{
      tiling/alignment~ edge=#1,
      tiling/alignment~ new~ edge=#2
    }
  },
  align~ between/.code~ args={#1~ and~ #2~ using~ #3}{
    \tikzset{
      tiling/alignment~ start={#1},
      tiling/alignment~ end={#2},
    }
    \str_set:Nn \l__tilings_tmpa_str {#3}
    \str_set:Nx \l__tilings_tmpb_str {\str_tail:N \l__tilings_tmpa_str}
    \tikzset{
      tiling/alignment~ new~ edge/.expanded={\str_use:N \l__tilings_tmpb_str}
    }
    \str_set:Nx \l__tilings_tmpa_str {\str_head:N \l__tilings_tmpa_str}
    \str_set:Nx \l__tilings_tmpb_str {\str_lowercase:f { \l__tilings_tmpa_str}}
    \str_if_eq:NNT \l__tilings_tmpa_str \l__tilings_tmpb_str
    {
      \str_set:Nx \l__tilings_tmpb_str
      {\str_uppercase:f { \l__tilings_tmpa_str}}
    }
    \tikzset{
      tiling/alignment~ edge/.expanded={\str_use:N \l__tilings_tmpb_str},
    }
  },
  tiling/alignment~ location/.initial={},
  tiling/alignment~ edge/.initial=a,
  tiling/alignment~ new~ edge/.initial={},
  tiling/alignment~ direction/.initial={forewards},
  tiling/alignment~ start/.initial={},
  tiling/alignment~ end/.initial={},
  tiling/anchor/.initial={},
  every~ tile~ clip/.style={clip}
}
\DeclareDocumentCommand \DefineTile { s m m m }
{
  \tl_clear:N \l__tilings_tmpa_tl
  \int_zero:N \l__tilings_tmpa_int
  \fp_zero:N \l__tilings_saved_x_fp
  \fp_zero:N \l__tilings_saved_y_fp
  \tl_map_inline:nn {#4} {
    \str_set:Nn \l__tilings_tmpa_str {##1}
    \str_if_eq:VnTF \l__tilings_tmpa_str {+}
    {
      \int_incr:N \l__tilings_tmpa_int
    }
    {
      \int_case:nn {\l__tilings_tmpa_int}
      {
        {0} {
          \bool_set_false:N \l__tilings_relative_bool
          \bool_set_true:N \l__tilings_update_saved_bool
        }
        {1} {
          \bool_set_true:N \l__tilings_relative_bool
          \bool_set_false:N \l__tilings_update_saved_bool
        }
        {2} {
          \bool_set_true:N \l__tilings_relative_bool
          \bool_set_true:N \l__tilings_update_saved_bool
        }

      }
      \str_if_in:NnTF \l__tilings_tmpa_str {:}
      {
        \seq_set_split:NVV \l__tilings_tmpa_seq \c__tilings_colon_str \l__tilings_tmpa_str
        \__tilings_add_coordinate:Nnn \l__tilings_tmpa_tl
        {
          (\seq_item:Nn \l__tilings_tmpa_seq {2}) * cosd (\seq_item:Nn \l__tilings_tmpa_seq {1})
        }
        {
          (\seq_item:Nn \l__tilings_tmpa_seq {2}) * sind (\seq_item:Nn \l__tilings_tmpa_seq {1})
        }
      }
      {
        \seq_set_split:NVV \l__tilings_tmpa_seq \c__tilings_comma_str \l__tilings_tmpa_str
        \__tilings_add_coordinate:Nnn \l__tilings_tmpa_tl
        {
          (\seq_item:Nn \l__tilings_tmpa_seq {1})
        }
        {
          (\seq_item:Nn \l__tilings_tmpa_seq {2})
        }
      }
      \int_zero:N \l__tilings_tmpa_int
    }
  }
  \prop_clear:N \l__tilings_tmpa_prop
  \tl_map_inline:nn {#3} {
    \prop_if_in:NnTF \l__tilings_tmpa_prop {##1}
    {
      \prop_put:Nnn \l__tilings_tmpa_prop {##1} {1}
    }
    {
      \prop_put:Nnn \l__tilings_tmpa_prop {##1} {0}
    }
  }
  \tl_clear:N \l__tilings_tmpb_tl
  \tl_map_inline:nn {#3}
  {
    \tl_clear:N \l__tilings_tmpc_tl
    \tl_put_right:Nn \l__tilings_tmpc_tl {##1}
    \int_compare:nF {\prop_item:Nn \l__tilings_tmpa_prop {##1} == 0} {
      \tl_put_right:Nx \l__tilings_tmpc_tl
      {\prop_item:Nn \l__tilings_tmpa_prop {##1}}
      \prop_put:Nnx \l__tilings_tmpa_prop {##1}
      {\int_eval:n {\prop_item:Nn \l__tilings_tmpa_prop {##1} + 1}}
    }
    \tl_put_right:Nx \l__tilings_tmpb_tl {{ \l__tilings_tmpc_tl }}
  }
  \prop_gput:Nnx \g__tilings_tiles_prop {#2}
  {{\tl_use:N \l__tilings_tmpb_tl} {\tl_use:N \l__tilings_tmpa_tl}}
  \tikzset{
    #2/.pic={
      \begin{scope}[
        every~ tile~ scope/.try,
        every~ #2~ scope/.try,
        this~ tile~ scope/.try
      ]
      \tikz@fig@mustbenamed
      \prop_gput:NVn \g__tilings_tilenames_prop \tikz@fig@name {#2}
      \__tilings_keys_get:Nn \l__tilings_tmpa_tl {alignment~ start}
      \tl_if_empty:NTF \l__tilings_tmpa_tl
      {
        \prop_get:NnN \g__tilings_tiles_prop {#2} \l__tilings_tmpa_tl
        \tl_set:Nx \l__tilings_tmpc_tl {\tl_head:N \l__tilings_tmpa_tl}
        \__tilings_keys_get:Nn \l__tilings_tmpa_tl {anchor}
        \tl_if_empty:NTF \l__tilings_tmpa_tl
        {
          \bool_if:NT \l__tilings_cw_bool
          {
            \pgftransformxscale {-1}
          }
        }
        {
          \regex_extract_once:NVNTF
          \c__tilings_anchor_regex \l__tilings_tmpa_tl \l__tilings_tmpb_tl
          {
            \regex_replace_once:NnN \c__tilings_anchor_regex {} \l__tilings_tmpa_tl
            \tl_if_eq:NnTF \l__tilings_tmpb_tl {~end}
            {
              \bool_set_true:N \l__tilings_cw_bool
            }
            {
              \bool_set_false:N \l__tilings_cw_bool
            }
          }
          {
            \bool_set_false:N \l__tilings_cw_bool
          }
          \tl_set:Nx \l__tilings_tmpb_tl {{\tl_use:N \l__tilings_tmpa_tl}}
          \tl_if_in:NVT \l__tilings_tmpc_tl \l__tilings_tmpb_tl
          {
            \__tilings_translate_vertex_to_origin:NnV
            \l__tilings_cw_bool {#2} \l__tilings_tmpa_tl
          }
        }
      }
      {
        \group_begin:
        \tikzset{
          name~ prefix~ ..
        }
        \tikz_scan_point:n {
          \__tilings_keys_get:n {alignment~ start}
        }
        \dim_set_eq:Nc \l__tilings_xa_dim {pgf@x}
        \dim_set_eq:Nc \l__tilings_ya_dim {pgf@y}
        \tikz_scan_point:n {
          \__tilings_keys_get:n {alignment~ end}
        }
        \dim_set_eq:Nc \l__tilings_xb_dim {pgf@x}
        \dim_set_eq:Nc \l__tilings_yb_dim {pgf@y}
        \__tilings_keys_get:Nn \l__tilings_tmpb_tl {alignment~ direction}
        \tl_if_eq:NnTF \l__tilings_tmpb_tl {forewards}
        {
          \dim_gset_eq:NN \g__tilings_xa_dim \l__tilings_xa_dim
          \dim_gset_eq:NN \g__tilings_ya_dim \l__tilings_ya_dim
          \dim_gset_eq:NN \g__tilings_xb_dim \l__tilings_xb_dim
          \dim_gset_eq:NN \g__tilings_yb_dim \l__tilings_yb_dim
        }
        {
          \dim_gset_eq:NN \g__tilings_xa_dim \l__tilings_xb_dim
          \dim_gset_eq:NN \g__tilings_ya_dim \l__tilings_yb_dim
          \dim_gset_eq:NN \g__tilings_xb_dim \l__tilings_xa_dim
          \dim_gset_eq:NN \g__tilings_yb_dim \l__tilings_ya_dim
        }
        \dim_gsub:Nn \g__tilings_xb_dim {\g__tilings_xa_dim}
        \dim_gsub:Nn \g__tilings_yb_dim {\g__tilings_ya_dim}
        \dim_gset:Nn \g__tilings_xb_dim {\g__tilings_xb_dim * \dim_ratio:nn {1pt}{1cm}}
        \dim_gset:Nn \g__tilings_yb_dim {\g__tilings_yb_dim * \dim_ratio:nn {1pt}{1cm}}
        \group_end:
        \pgftransformshift{\pgfpoint{\g__tilings_xa_dim}{\g__tilings_ya_dim}}
        \pgftransformtriangle
        {\pgfpoint{0pt}{0pt}}
        {\pgfpoint{\g__tilings_xb_dim}{\g__tilings_yb_dim}}
        {\pgfpoint{-\g__tilings_yb_dim}{\g__tilings_xb_dim}}
        \str_set:Nx \l__tilings_tmpa_str
        {\__tilings_keys_get:n {alignment~ edge}}
        \str_set:Nx \l__tilings_tmpa_str {\str_head:N \l__tilings_tmpa_str}
        \str_put_right:Nx \l__tilings_tmpa_str
        {\__tilings_keys_get:n {alignment~ new~ edge}}
        \str_set:Nx \l__tilings_tmpb_str {\str_lowercase:f { \l__tilings_tmpa_str}}
        \str_if_eq:NNT \l__tilings_tmpa_str \l__tilings_tmpb_str
        {
          \str_set:Nx \l__tilings_tmpb_str
          {\str_uppercase:f { \l__tilings_tmpa_str}}
        }

        \IfBooleanT {#1}
        {
          \bool_set:Nn \l__tilings_cw_bool {!\l__tilings_cw_bool}
        }
        \bool_if:NT \l__tilings_cw_bool
        {
          \pgftransformyscale {-1}
        }
        \__tilings_transform_side_to_axis:NnV \l__tilings_cw_bool {#2} \l__tilings_tmpb_str
      }
      \__tilings_coordinates_at_vertices:n {#2}
      \coordinate[alias=-center] (-centre) at (0,0);
      \UseTile[
        every~ tile~ clip/.try,
        every~ #2~ clip/.try,
        this~ tile~ clip/.try
      ]{#2}
      \tikzset{
        every~ tile~ before~ path/.try,
        every~ #2~ before~ path/.try,
        this~ tile~ before~ path/.try
      }
      \UseTile[
        every~ tile/.try,
        every~ #2/.try,
        this~ tile/.try,
        pic~ actions
      ]{#2}
      \tikzset{
        every~ tile~ after~ path/.try,
        every~ #2~ after~ path/.try,
        this~ tile~ after~ path/.try
      }
      \end{scope}
    },
    #2/.style={
      every~ tile~ pic/.try,
      every~ #2~ pic/.try,
      pic~ type=#2,
    }
  }
}
\cs_new_protected_nopar:Npn \__tilings_bake_tile:n #1
{
  \prop_get:NnN \g__tilings_tiles_prop {#1} \l__tilings_tmpa_tl
  \__tilings_make_tile:nV {#1} \l__tilings_tmpa_tl
}

\NewDocumentCommand \BakeTile {m}
{
  \__tilings_bake_tile:n {#1}
}
\cs_new_protected_nopar:Npn \__tilings_use_tile:nn #1#2
{
  \tl_if_exist:cTF {g__tilings_tile_#2_tl}
  {
    \tl_set_eq:Nc \l__tilings_tmp_tile_path_tl {g__tilings_tile_#2_tl}
    \pgfgettransform \l__tilings_tmpa_tl
    \spath_transform:NV \l__tilings_tmp_tile_path_tl \l__tilings_tmpa_tl
    \spath_tikz_path:nV {#1} \l__tilings_tmp_tile_path_tl
  }
  {
    \msg_error:nnn { tilings }{ not baked }{#2}
  }
}

\NewDocumentCommand \UseTile {O{} m}
{
  \__tilings_use_tile:nn {#1}{#2}
}
\tikzset{
  save~ tiling~ path/.code={
    \tikz@addmode{
      \pgfsyssoftpath@getcurrentpath\l__tilings_tmpa_tl
      \__tilings_normalise_path:N \l__tilings_tmpa_tl
      \tl_gclear_new:c {g__tilings_side_#1_tl}
      \tl_gset_eq:cN {g__tilings_side_#1_tl} \l__tilings_tmpa_tl
      \tl_set:Nx \l__tilings_tmpb_tl {\str_uppercase:n {#1}}
      \spath_reverse:N \l__tilings_tmpa_tl
      \spath_transform:Nnnnnnn \l__tilings_tmpa_tl {-1} {0} {0} {-1} {1} {0}
      \tl_gclear_new:c {g__tilings_side_ \tl_use:N \l__tilings_tmpb_tl _tl}
      \tl_gset_eq:cN {g__tilings_side_ \tl_use:N \l__tilings_tmpb_tl _tl} \l__tilings_tmpa_tl
    }
  },
  clone~ tiling~ side~ path/.style~ 2~ args={
    spath/set~ name=tiling~ side,
    spath/clone~ global={#1}{#2}
  },
  flip~ tile/.code={
    \tl_set:Nn \l__tilings_tmpa_tl {#1}
    \tl_set:Nn \l__tilings_tmpb_tl {true}
    \bool_set:Nn \l__tilings_cw_bool {\tl_if_eq_p:NN \l__tilings_tmpa_tl \l__tilings_tmpb_tl}
  },
  flip~ tile/.default={true},
  spath/prefix/tiling~side/.style={
    spath/set~ prefix=g__tilings_side_,
  },
  spath/suffix/tiling~side/.style={
    spath/set~ suffix=_tl,
  },
  clone~ tile~ path/.style~ 2~ args={
    spath/set~ name=tiling~tile,
    spath/clone~ global={#1}{#2}
  },
  spath/prefix/tiling~tile/.style={
    spath/set~ prefix=g__tilings_tile_,
  },
  spath/suffix/tiling~tile/.style={
    spath/set~ suffix=_tl,
  },
  expand~ key/.code={
    \exp_args:NV \pgfkeysalso #1
  }
}
\cs_new_nopar:Npn \__tilings_make_lms:Nnnn #1#2#3#4
{
  \group_begin:
  \tl_set:Nn \l__tilings_tmpb_tl {#4}
  \prg_replicate:nn {#3} {
    \tl_set_eq:NN \l__tilings_tmpa_tl \l__tilings_tmpb_tl
    \tl_clear:N \l__tilings_tmpb_tl
    \tl_map_inline:Nn \l__tilings_tmpa_tl
    {
      \tl_set:Nx \l__tilings_action_lms_tl {\tl_head:n {##1}}
      \tl_set:Nx \l__tilings_parameters_lms_tl {\tl_tail:n {##1}}
      \prop_if_in:cVTF {g__tilings_#2_lms_rule_prop} \l__tilings_action_lms_tl
      {
        \prop_get:cVN {g__tilings_#2_lms_rule_prop} \l__tilings_action_lms_tl \l__tilings_tmpc_tl
        \tl_put_right:Nx \l__tilings_tmpb_tl {\tl_use:N \l__tilings_tmpc_tl}
      }
      {
        \tl_if_single:nTF {##1}
        {
          \tl_put_right:Nn \l__tilings_tmpb_tl {##1}
        }
        {
          \tl_put_right:Nn \l__tilings_tmpb_tl {{##1}}
        }
      }
    }
  }
  \tl_set:Nn \l__tilings_tmpa_tl {
    \group_end:
    \tl_set:Nn #1
  }
  \tl_put_right:Nx \l__tilings_tmpa_tl {{\tl_use:N \l__tilings_tmpb_tl}}
  \tl_use:N \l__tilings_tmpa_tl
}
\cs_generate_variant:Nn \__tilings_make_lms:Nnnn {Nnnx}
\cs_new_nopar:Npn \__tilings_invoke_lms:nn #1#2
{
  \group_begin:
  \tl_map_inline:nn {#1} {
    \tl_set:Nx \l__tilings_action_lms_tl {\tl_head:n {##1}}
    \tl_set:Nx \l__tilings_parameters_lms_tl {\tl_tail:n {##1}}
    \prop_if_in:cVTF {g__tilings_#2_lms_action_prop} \l__tilings_action_lms_tl
    {
      \prop_item:cV {g__tilings_#2_lms_action_prop} \l__tilings_action_lms_tl
    }
    {
      \prop_if_in:cVT {g__tilings_default_lms_action_prop} \l__tilings_action_lms_tl
      {
        \prop_item:cV {g__tilings_default_lms_action_prop} \l__tilings_action_lms_tl
      }
    }
  }
  \group_end:
}
\cs_generate_variant:Nn \__tilings_invoke_lms:nn {Vn}
\dim_new:N \l__tilings_step_dim
\dim_set:Nn \l__tilings_step_dim {1cm}
\prop_new:N \g__tilings_default_lms_action_prop
\prop_gput:Nnn \g__tilings_default_lms_action_prop {[} {\group_begin:}
\prop_gput:Nnn \g__tilings_default_lms_action_prop {]} {\group_end:}
\prop_gput:Nnn \g__tilings_default_lms_action_prop {f}
{\pgftransformxshift{\l__tilings_step_dim}}
\prop_gput:Nnn \g__tilings_default_lms_action_prop {b}
{\pgftransformxshift{-\l__tilings_step_dim}}
\prop_new:N \g__tilings_drawables_lms_prop
\int_new:N \g__tilings_tile_int
\int_new:N \g__tilings_tiles_int
\cs_new_protected_nopar:Npn \__tilings_tiling_decomposition:nnnn #1#2#3#4
{
  \group_begin:
  \tikzset{
    every~ #2~ decomposition/.try,
    #1
  }
  \__tilings_make_lms:Nnnx \l__tilings_tmpa_tl {#2} {#3} {#4}
  \__tilings_count_lms:Vn \l__tilings_tmpa_tl {#2}
  \int_gzero:N \g__tilings_tile_int
  \__tilings_invoke_lms:Vn \l__tilings_tmpa_tl {#2}
  \group_end:
}
\cs_new_protected_nopar:Npn \__tilings_tiling_decomposition:nnn #1#2#3
{
  \__tilings_tiling_decomposition:nnnn {}{#1}{#2}{#3}
}
\cs_generate_variant:Nn \__tilings_tiling_decomposition:nnn {VVV}

\NewDocumentCommand \TilingDecomposition { O{} m m m }
{
 \__tilings_tiling_decomposition:nnnn {#1}{#2}{#3}{#4}
}

\tikzset{
  pics/decomposition/.style~ n~ args={3}{
    code={
      \__tilings_tiling_decomposition:nnn {#1}{#2}{#3}
    }
  }
}
\cs_new_nopar:Npn \__tilings_count_lms:nn #1#2
{
  \group_begin:
  \int_gzero:N \g__tilings_tiles_int
  \prop_get:NnNT \g__tilings_drawables_lms_prop {#2} \l__tilings_tmpa_tl
  {
    \tl_map_variable:nNn {#1} \l__tilings_tmpb_tl
    {
      \tl_set:Nx \l__tilings_tmpb_tl {\tl_head:N \l__tilings_tmpb_tl}
      \bool_do_while:nn
      {
        !\tl_if_empty_p:N \l__tilings_tmpb_tl
        &&
        \tl_if_head_is_group_p:V \l__tilings_tmpb_tl
      }
      {
        \tl_set:Nx \l__tilings_tmpb_tl {\tl_head:N \l__tilings_tmpb_tl}
      }
      \tl_if_in:NVT \l__tilings_tmpa_tl \l__tilings_tmpb_tl
      {
        \int_gincr:N \g__tilings_tiles_int
      }
    }
  }
  \group_end:
}
\cs_generate_variant:Nn \__tilings_count_lms:nn {Vn}
\tikzset{
  tiling~ step/.code={
    \dim_set:Nn \l__tilings_step_dim {#1}
  }
}
\ExplSyntaxOff
%% 
%% Copyright (C) 2014-2023 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  penrose_code.dtx
%%                                  penrose.tex
%% and the derived files            penrose.ins
%%                                  penrose_code.pdf
%%                                  penrose.pdf
%%                                  tikzlibrarytilings.code.tex
%%                                  tikzlibrarytilings.penrose.code.tex
%%                                  tikzlibrarytilings.polykite.code.tex
%%                                  tikzlibrarypenrose.code.tex
%%                                  README.txt
%% 
%%
%% End of file `tikzlibrarytilings.code.tex'.


==> tikzlibrarytilings.penrose.code.tex <==
%%
%% This is file `tikzlibrarytilings.penrose.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tilings_code.dtx  (with options: `penrose')
%% ----------------------------------------------------------------
%% tilings --- TikZ library for producing tilings
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\RequirePackage{tikz}
\usetikzlibrary{tilings}
\ProvidesFile {tikzlibrarytilings.penrose.code.tex}
[2023/06/01 v2.0 TikZ pics for Penrose tiles]
\DefineTile{thin rhombus}{a A B b}
{
 {0 , 0}
 {cosd(18) , sind(18)}
 {2*cosd(18) , 0}
 {cosd(18) , -sind(18)}
}
\DefineTile{thick rhombus}{B a A b}
{
 {0 , 0}
 {cosd(36) , sind(36)}
 {2*cosd(36) , 0}
 {cosd(36) , -sind(36)}
}
\DefineTile{dart}{c a A C}
{
 {0 , 0}
 {2*sind(18)*cosd(108) , 2*sind(18)*sind(108)}
 {2*sind(18) , 0}
 {2*sind(18)*cosd(108) , -2*sind(18)*sind(108)}
}
\DefineTile{kite}{a c C A}
{
 {0 , 0}
 {cosd(36) , sind(36)}
 {1 , 0}
 {cosd(36) , -sind(36)}
}
\DefineTile{golden triangle}{a c b}
{
 {0 , 0}
 {cosd(18) , sind(18)}
 {cosd(18) , -sind(18)}
}
\DefineTile {reverse golden triangle}{B C A}
{
 {0 , 0}
 {cosd(18) , sind(18)}
 {cosd(18) , -sind(18)}
}
\DefineTile {golden gnomon}{C b A}
{
 {0 , 0}
 {cosd(36) , sind(36)}
 {2*cosd(36) , 0}
}
\DefineTile {reverse golden gnomon}{a B c}
{
 {0 , 0}
 {2*cosd(36) , 0}
 {cosd(36) , -sind(36)}
}
\DefineTile {pentagon 5}{a a a a a}
{
 {0 , 0}
 {cosd(108) , sind(108)}
 {1+cosd(72)+cosd(144) , sind(72)+sind(144)}
 {1+cosd(72) , sind(72)}
 {1 , 0}
}
\DefineTile {pentagon 3}{A b a a b}
{
 {0 , 0}
 {cosd(108) , sind(108)}
 {1+cosd(72)+cosd(144) , sind(72)+sind(144)}
 {1+cosd(72) , sind(72)}
 {1 , 0}
}
\DefineTile {pentagon 2}{d A e c A}
{
 {0 , 0}
 {cosd(108) , sind(108)}
 {1+cosd(72)+cosd(144) , sind(72)+sind(144)}
 {1+cosd(72) , sind(72)}
 {1 , 0}
}
\DefineTile {pentagram}{C E C E C E C E C E}
{
  {1 , 0}
  {1-cosd(36) , -sind(36)}
  {1-cosd(36)-cosd(108) , -sind(36)-sind(108)}
  {cosd(108) , -sind(108)}
  {-1+3*cosd(108)+cosd(36) , -sind(36)-sind(108)}
  {-1+2*cosd(108)+cosd(36) , -sind(36)}
  {-1+2*cosd(108) , 0}
  {2*cosd(108) , 0}
  {cosd(108) , sind(108)}
  {0 , 0}
}
\DefineTile {boat}{C E C E B D B}
{
 {-1+2*cosd(108) , 0}
 {2*cosd(108) , 0}
 {cosd(108) , sind(108)}
 {0 , 0}
 {1 , 0}
 {1-cosd(36) , -sind(36)}
 {-1+2*cosd(108)+cosd(36) , -sind(36)}
}
\DefineTile {diamond}{D B B D}
{
 {0 , 0}
 {cosd(18) , sind(18)}
 {2*cosd(18) , 0}
 {cosd(18) , -sind(18)}
}
\tikzset{
  every thin rhombus before path/.code={
    \path[every circle arc/.try] (-edge a end) circle[radius=1/4];
    \path[every long arc/.try] (-edge b start) circle[radius=1/4];
  },
  every thick rhombus before path/.code={
    \path[every circle arc/.try] (-edge a end) circle[radius=1/4];
    \path[every long arc/.try] (-edge B start) circle[radius=3/4];
  },
  every kite before path/.code={
    \path[every circle arc/.try] (-edge a start) circle[radius=2/(sqrt(5)+1)];
    \path[every long arc/.try] (-edge c end) circle[radius=2/(3+sqrt(5))];
  },
  every dart before path/.code={
    \path[every circle arc/.try] (-edge a end) circle[radius=1 - 2/(sqrt(5)+1)];
    \path[every long arc/.try] (-edge c start) circle[radius=2/(sqrt(5)+1) - 2/(3+sqrt(5))];
  }
}
\BakeTile {thin rhombus}
\BakeTile {thick rhombus}
\BakeTile {dart}
\BakeTile {kite}
\BakeTile {golden triangle}
\BakeTile {reverse golden triangle}
\BakeTile {golden gnomon}
\BakeTile {reverse golden gnomon}
\BakeTile {pentagon 5}
\BakeTile {pentagon 3}
\BakeTile {pentagon 2}
\BakeTile {pentagram}
\BakeTile {boat}
\BakeTile {diamond}
\ExplSyntaxOn
\prop_new:N \g__tilings_rhombus_lms_rule_prop
\prop_gput:Nnn \g__tilings_rhombus_lms_rule_prop {T} {[f*sT][f>g]}
\prop_gput:Nnn \g__tilings_rhombus_lms_rule_prop {t} {[f_st][f>G]}
\prop_gput:Nnn \g__tilings_rhombus_lms_rule_prop {G} {[f+sG][sf>g][sf*sT]}
\prop_gput:Nnn \g__tilings_rhombus_lms_rule_prop {g} {[f-sg][sf>G][sf_st]}
\prop_new:N \g__tilings_kite_lms_rule_prop
\prop_gput:Nnn \g__tilings_kite_lms_rule_prop {T} {[f*sT][f>st][+sg]}
\prop_gput:Nnn \g__tilings_kite_lms_rule_prop {t} {[f_st][f>sT][-sG]}
\prop_gput:Nnn \g__tilings_kite_lms_rule_prop {G} {[f*+sG][sT]}
\prop_gput:Nnn \g__tilings_kite_lms_rule_prop {g} {[f-_sg][st]}
\prop_new:N \g__tilings_pentagon_lms_rule_prop
\prop_gput:Nnn \g__tilings_pentagon_lms_rule_prop {P}
{[s>P][1sF+Q][1+sF+Q][1*sF+Q][1-sF+Q][1_sF+Q]} % pentagon 5
\prop_gput:Nnn \g__tilings_pentagon_lms_rule_prop {Q}
{[s>P][1+sFR][1*sF*R][1-sF+Q][1_sF+Q][1sF+Q][->fsD]} % pentagon 3
\prop_gput:Nnn \g__tilings_pentagon_lms_rule_prop {R}
{[s>P][1-sF+Q][1+sF*R][1*sFR][1_sF*R][1sFR][_>fsD][>fsD]} % pentagon 2
\prop_gput:Nnn \g__tilings_pentagon_lms_rule_prop {G}
{
  [s>G]
  [se[>d+R][e1B]]
  [+se[>d+R][e1B]]
  [-se[>d+R][e1B]]
  [*se[>d+R][e1B]]
  [_se[>d+R][e1B]]
} % pentagram
\prop_gput:Nnn \g__tilings_pentagon_lms_rule_prop {B}
{
  [s>G]
  [se[>d+R][e1B]]
  [+se[>d+R][e1B]]
  [-se[>d+R][e1B]]
} % boat
\prop_gput:Nnn \g__tilings_pentagon_lms_rule_prop {D}
{[s>d+R][s>eG][se1B]} % diamond
\prop_gset_eq:NN \g__tilings_rtriangle_lms_rule_prop
\g__tilings_rhombus_lms_rule_prop
\prop_gset_eq:NN \g__tilings_ktriangle_lms_rule_prop
\g__tilings_kite_lms_rule_prop
\prop_gput:Nnn \g__tilings_drawables_lms_prop {rhombus} {TG}
\prop_gput:Nnn \g__tilings_drawables_lms_prop {kite} {Tg}
\prop_gput:Nnn \g__tilings_drawables_lms_prop {rtriangle} {TtGg}
\prop_gput:Nnn \g__tilings_drawables_lms_prop {ktriangle} {TtGg}
\prop_gput:Nnn \g__tilings_drawables_lms_prop {pentagon} {PQRGBD}
\prop_new:N \g__tilings_rhombus_lms_action_prop
\prop_new:N \g__tilings_kite_lms_action_prop
\prop_new:N \g__tilings_rtriangle_lms_action_prop
\prop_new:N \g__tilings_ktriangle_lms_action_prop
\prop_new:N \g__tilings_pentagon_lms_action_prop
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {+}
{\pgftransformrotate{144}}
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {*}
{\pgftransformrotate{108}}
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {-}
{\pgftransformrotate{216}}
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {_}
{\pgftransformrotate{252}}
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {>}
{\pgftransformrotate{180}}
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {s} {
  \fp_set:Nn \l__tilings_tmpa_fp { 2 * sind(18) * \l__tilings_step_dim }
  \dim_set:Nn \l__tilings_step_dim {\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gset_eq:NN \g__tilings_rtriangle_lms_action_prop
\g__tilings_rhombus_lms_action_prop
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {T} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{198}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*2*cosd(18)}
  \pgftransformxshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ thin~ rhombus/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{thin~rhombus}
  \group_end:
}
\prop_gput:Nnn \g__tilings_rhombus_lms_action_prop {G} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)/(2*cosd(36))}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ thick~ rhombus/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{thick~rhombus}
  \group_end:
}
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {+} {\pgftransformrotate{36}}
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {*} {\pgftransformrotate{108}}
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {-} {\pgftransformrotate{-36}}
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {_}
{\pgftransformrotate{-108}}
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {>} {\pgftransformrotate{180}}
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {s} {
  \fp_set:Nn \l__tilings_tmpa_fp { 2 * sind(18) * \l__tilings_step_dim }
  \dim_set:Nn \l__tilings_step_dim {\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gset_eq:NN \g__tilings_ktriangle_lms_action_prop
\g__tilings_kite_lms_action_prop
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {T} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{36}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ kite/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{kite}
  \group_end:
}
\prop_gput:Nnn \g__tilings_kite_lms_action_prop {g} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{144}
  \pgftransformxshift{-\l__tilings_step_dim * 2 * sin(18)}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ dart/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{dart}
  \group_end:
}
\prop_gput:Nnn \g__tilings_rtriangle_lms_action_prop {T} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{18}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ reverse~ golden~ triangle/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{reverse~ golden~ triangle}
  \group_end:
}
\prop_gput:Nnn \g__tilings_rtriangle_lms_action_prop {t} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{-18}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ golden~ triangle/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{golden~ triangle}
  \group_end:
}
\prop_gput:Nnn \g__tilings_rtriangle_lms_action_prop {G} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{180}
  \pgftransformxshift{-\l__tilings_step_dim}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)/(2*cosd(36))}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ reverse~ golden~ gnomon/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{reverse~ golden~ gnomon}
  \group_end:
}
\prop_gput:Nnn \g__tilings_rtriangle_lms_action_prop {g} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{180}
  \pgftransformxshift{-\l__tilings_step_dim}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)/(2*cosd(36))}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ golden~ gnomon/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{golden~ gnomon}
  \group_end:
}
\prop_gput:Nnn \g__tilings_ktriangle_lms_action_prop {T} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{18}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ reverse~ golden~ triangle/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{reverse~ golden~ triangle}
  \group_end:
}
\prop_gput:Nnn \g__tilings_ktriangle_lms_action_prop {t} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{-18}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ golden~ triangle/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{golden~ triangle}
  \group_end:
}
\prop_gput:Nnn \g__tilings_ktriangle_lms_action_prop {G} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{180}
  \pgftransformxshift{-\l__tilings_step_dim}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)/(2*cosd(36))}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ reverse~ golden~ gnomon/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{reverse~ golden~ gnomon}
  \group_end:
}
\prop_gput:Nnn \g__tilings_ktriangle_lms_action_prop {g} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{180}
  \pgftransformxshift{-\l__tilings_step_dim}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)/(2*cosd(36))}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ golden~ gnomon/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{golden~ gnomon}
  \group_end:
}
\int_new:N \l__tilings_pentagon_parity_int
\seq_new:N \l__tilings_pentagon_parity_seq
\seq_set_from_clist:Nn \l__tilings_pentagon_parity_seq {odd,even}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {1} {
  \int_set:Nn \l__tilings_pentagon_parity_int
  {3 -  \l__tilings_pentagon_parity_int}
}
\tikzset{
  every~ pentagon~ decomposition/.code={%
    \int_set:Nn \l__tilings_pentagon_parity_int {2}
  }
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {+}
{\pgftransformrotate{72}}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {*}
{\pgftransformrotate{144}}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {-}
{\pgftransformrotate{288}}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {_}
{\pgftransformrotate{216}}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {>}
{\pgftransformrotate{180}}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {|}
{\pgftransformxscale{-1}}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {s} {
  \fp_set:Nn \l__tilings_tmpa_fp
  {
    1/(2 + 2 * cosd(72) ) * \l__tilings_step_dim
  }
  \dim_set:Nn \l__tilings_step_dim {\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {f} {
  \fp_set:Nn \l__tilings_tmpa_fp {  tand(54)/2 * \l__tilings_step_dim }
  \pgftransformyshift{\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {F} {
  \fp_set:Nn \l__tilings_tmpa_fp {  tand(54) * \l__tilings_step_dim }
  \pgftransformyshift{\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {d} {
  \fp_set:Nn \l__tilings_tmpa_fp
  {
    (tand(54)/2 - tand(72)/2 + sind(36) ) * \l__tilings_step_dim
  }
  \pgftransformyshift{\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {e} {
  \fp_set:Nn \l__tilings_tmpa_fp
  {
    tand(54) * cosd(36) * \l__tilings_step_dim
  }
  \pgftransformyshift{\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {P} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/2}
  \pgftransformxshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*tand(54)/2}
  \pgftransformyshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ pentagon/.try,
    every~
    \seq_item:Nn \l__tilings_pentagon_parity_seq
    {\l__tilings_pentagon_parity_int}
    \space pentagon/.try,
    every~ pentagon~ 5/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{pentagon~5}
  \group_end:
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {Q} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/2}
  \pgftransformxshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*tand(54)/2}
  \pgftransformyshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ pentagon/.try,
    every~
    \seq_item:Nn \l__tilings_pentagon_parity_seq
    {\l__tilings_pentagon_parity_int}
    \space pentagon/.try,
    every~ pentagon~ 3/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{pentagon~3}
  \group_end:
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {R} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/2}
  \pgftransformxshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*tand(54)/2}
  \pgftransformyshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ pentagon/.try,
    every~
    \seq_item:Nn \l__tilings_pentagon_parity_seq
    {\l__tilings_pentagon_parity_int}
    \space pentagon/.try,
    every~ pentagon~ 2/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{pentagon~2}
  \group_end:
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {G} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*cosd(72)}
  \pgftransformxshift{\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*tand(54)*cosd(72)}
  \pgftransformyshift{\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ pentagram/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{pentagram}
  \group_end:
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {B} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*cosd(72)}
  \pgftransformxshift{\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*tand(54)*cosd(72)}
  \pgftransformyshift{\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ boat/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{boat}
  \group_end:
}
\prop_gput:Nnn \g__tilings_pentagon_lms_action_prop {D} {
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \pgftransformrotate{90}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim*cosd(18)}
  \pgftransformxshift{-\fp_to_dim:N \l__tilings_tmpa_fp}
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ diamond/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{diamond}
  \group_end:
}
\ExplSyntaxOff
%% 
%% Copyright (C) 2014-2023 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  penrose_code.dtx
%%                                  penrose.tex
%% and the derived files            penrose.ins
%%                                  penrose_code.pdf
%%                                  penrose.pdf
%%                                  tikzlibrarytilings.code.tex
%%                                  tikzlibrarytilings.penrose.code.tex
%%                                  tikzlibrarytilings.polykite.code.tex
%%                                  tikzlibrarypenrose.code.tex
%%                                  README.txt
%% 
%%
%% End of file `tikzlibrarytilings.penrose.code.tex'.


==> tikzlibrarytilings.polykite.code.tex <==
%%
%% This is file `tikzlibrarytilings.polykite.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tilings_code.dtx  (with options: `polykite')
%% ----------------------------------------------------------------
%% tilings --- TikZ library for producing tilings
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\RequirePackage{tikz}
\usetikzlibrary{tilings}
\ProvidesFile {tikzlibrarytilings.polykite.code.tex}
 [2023/06/01 v2.0 TikZ pics for Aperiodical Polykite tiles]
\DeclareDocumentCommand \DefinePolykiteTile {s m m m}
{
  \IfBooleanTF {#1}
  {
    \DefineTile {#2} {2 2 1 1 2 2 1 1 1 1 2 2 1 1}
  }
  {
    \DefineTile {#2} {1 1 2 2 1 1 2 2 2 2 1 1 2 2}
  }
  {
    {0 : #4}
    ++{90 : #3}
    ++{150 : #3}
    ++{240 : #4}
    ++{180 : #4}
    ++{-90 : #3}
    ++{210 : #3}
    ++{-60 : #4}
    ++{0 : #4}
    ++{0 : #4}
    ++{60 : #4}
    ++{-30 : #3}
    ++{30 : #3}
    ++{120 : #4}
  }
}
\DefinePolykiteTile{aperiodical hat}{sqrt(3)/2}{1/2}
\DefinePolykiteTile{spectral hat}{sqrt(3)/2}{1/2}
\DefinePolykiteTile{aperiodical turtle}{1/2}{sqrt(3)/2}
\DefinePolykiteTile*{spectral turtle}{1/2}{sqrt(3)/2}
\DefineTile {spectre} {a A a A a A a A a A a A a A}
  {
    {0 : .75}
    ++{90 : .75}
    ++{150 : .75}
    ++{240 : .75}
    ++{180 : .75}
    ++{-90 : .75}
    ++{210 : .75}
    ++{-60 : .75}
    ++{0 : .75}
    ++{0 : .75}
    ++{60 : .75}
    ++{-30 : .75}
    ++{30 : .75}
    ++{120 : .75}
  }
\DefineTile{meta cluster T}{A A b}
{
{ -1.5 , -sqrt(3)/2 }
{  1.5 , -sqrt(3)/2 }
{  0   ,  sqrt(3) }
}
\DefineTile{meta cluster P}{1 D d A 1 D d b}
{
{ -2.5, sqrt(3)/2 }
{ -2, 0 }
{ -1.5, -sqrt(3)/2 }
{ -0.5 , -sqrt(3)/2 }
{  2.5 , -sqrt(3)/2 }
{  2 , 0 }
{ 1.5 , sqrt(3)/2 }
{ .5 , sqrt(3)/2 }
}
\DefineTile{meta cluster F}{1 D d 1 D c C d b}
{
{ -2.5, sqrt(3)/2 }
{ -2, 0 }
{ -1.5, -sqrt(3)/2 }
{ -0.5 , -sqrt(3)/2 }
{ .5 , -sqrt(3)/2 }
{ 1.5 , -sqrt(3)/2 }
{  2 , 0 }
{ 1.5 , sqrt(3)/2 }
{ .5 , sqrt(3)/2 }
}
\DefineTile{meta cluster H}{B D d B D d a D d}
{
{ -2, -sqrt(3) }
{ 1, -sqrt(3) }
{ 2, -sqrt(3) }
{ 2.5, -sqrt(3)/2 }
{ 1, sqrt(3)}
{ .5 , 3*sqrt(3)/2 }
{ -.5 , 3*sqrt(3)/2 }
{ -2, 0 }
{ -2.5, -sqrt(3)/2 }
}
\DefineTile{super cluster T}{A A b}
{
{ -30 : 3 * (1 + sqrt(5))/2 / sqrt(3) }
{ 90 : 3 * (1 + sqrt(5))/2 / sqrt(3) }
{ 210 : 3 * (1 + sqrt(5))/2 / sqrt(3) }
}
\DefineTile{super cluster P}{1 D d A 1 D d b}
{
{ - 1.75 - sqrt(5), (sqrt(5)/2 + 1) * sqrt(3)/2 }
++{ -60 : 1 + sqrt(5) }
++{ -60 : 1}
++{ 1, 0}
++{ 3*(1 + sqrt(5))/2, 0 }
++{ 120 : 1 + sqrt(5) }
++{ 120 : 1 }
++{ -1, 0 }
}
\DefineTile{super cluster F}{1 D d 1 D c C d b}
{
{ - 1.75 - sqrt(5), (sqrt(5)/2 + 1) * sqrt(3)/2 }
++{ -60 : 1 + sqrt(5) }
++{ -60 : 1}
++{ 1, 0}
++{ 1 + sqrt(5), 0 }
++{ 1, 0 }
+{ -.75 + (2 + sqrt(5)) * sqrt(3)/4 * sqrt(3)/3,
  (2 + sqrt(5)) * sqrt(3)/4 + 3/4 * sqrt(3)/3 }
++{ -1.5, (2 + sqrt(5)) * sqrt(3)/2 }
++{ -1, 0 }
}
\DefineTile{super cluster H}{B D d B D d a D d}
{
{1.75 + 3*sqrt(5)/4, -(1 + sqrt(5))*sqrt(3)/4}
++{120 : 3*(1+sqrt(5))/2 }
++{120 : 1 }
++{-1,0}
++{240 : 3*(1+sqrt(5))/2}
++{240 : 1}
++{300 : 1}
++{ 3*(1+sqrt(5))/2, 0 }
++{1, 0}
++{60 : 1}
}
\DefineTile{subcluster H}{B B a}
{
  { 0, 0 }
  { 3, 0 }
  { 60 : 3 }
}
\DefineTile{subcluster T}{A A b}
{
  { 0, 0 }
  { 3, 0 }
  { 60 : 3 }
}
\DefineTile{subcluster P}{ 1 A 1 b }
{
  { 0, 0 }
  { 1, 0 }
  { 4, 0 }
  { 3, 0 }
}
\DefineTile{subcluster F}{ 1 1 f F b }
{
  { 0, 0 }
  { 1, 0 }
  +{ 60 : 1 }
  { 2, 0 }
  { 3, 0 }
}
\tikzset{
  no clip/.code={%
    \tikz@addmode{\tikz@mode@clipfalse}%
  },
  every subcluster P clip/.style={no clip},
  every subcluster F clip/.style={no clip},
}
\BakeTile {aperiodical hat}
\BakeTile {aperiodical turtle}
\BakeTile {spectral hat}
\BakeTile {spectral turtle}
\BakeTile {spectre}
\BakeTile {meta cluster T}
\BakeTile {meta cluster P}
\BakeTile {meta cluster F}
\BakeTile {meta cluster H}
\BakeTile {super cluster T}
\BakeTile {super cluster P}
\BakeTile {super cluster F}
\BakeTile {super cluster H}
\ExplSyntaxOn
\clist_map_inline:nn {a,A,b,B,f,F}
{
  \tl_new:c {g__tilings_side_polykite_#1_tl}
  \tl_if_exist:cF {g__tilings_side_#1_tl}
  {
    \tl_new:c {g__tilings_side_#1_tl}
  }
}

\tl_gset:cn {g__tilings_side_polykite_A_tl}
{
  \pgfsyssoftpath@movetotoken {0pt}{-0.3333332942822268pt}
  \pgfsyssoftpath@linetotoken {0.0833331478405773pt}{-0.1889954840909892pt}
  \pgfsyssoftpath@linetotoken {0.3333332942822268pt}{-0.3333332942822268pt}
  \pgfsyssoftpath@linetotoken {0.5833333235705567pt}{-0.1889954840909892pt}
  \pgfsyssoftpath@linetotoken {0.6666667057177732pt}{-0.3333332942822268pt}
  \pgfsyssoftpath@linetotoken {1pt}{-0.3333332942822268pt}
}
\tl_gset:cn {g__tilings_side_polykite_a_tl}
{
  \pgfsyssoftpath@movetotoken {0pt}{0.33333pt}
  \pgfsyssoftpath@linetotoken {0.33333pt}{0.33333pt}
  \pgfsyssoftpath@linetotoken {0.41667pt}{0.189pt}
  \pgfsyssoftpath@linetotoken {0.66667pt}{0.33333pt}
  \pgfsyssoftpath@linetotoken {0.91667pt}{0.189pt}
  \pgfsyssoftpath@linetotoken {1pt}{0.33333pt}
}
\tl_gset:cn {g__tilings_side_polykite_B_tl}
{
  \pgfsyssoftpath@movetotoken {0pt}{0pt}
  \pgfsyssoftpath@linetotoken {0.3333332942822268pt}{0pt}
  \pgfsyssoftpath@linetotoken {0.4166665592761237pt}{0.1443378101912376pt}
  \pgfsyssoftpath@linetotoken {0.6666667057177732pt}{0pt}
  \pgfsyssoftpath@linetotoken {0.9166666178527835pt}{0.1443378101912376pt}
  \pgfsyssoftpath@linetotoken {1pt}{0pt}
}
\tl_gset:cn {g__tilings_side_polykite_b_tl}
{
  \pgfsyssoftpath@movetotoken {0pt}{0pt}
  \pgfsyssoftpath@linetotoken {0.08333pt}{-0.14433pt}
  \pgfsyssoftpath@linetotoken {0.33333pt}{0pt}
  \pgfsyssoftpath@linetotoken {0.58333pt}{-0.14433pt}
  \pgfsyssoftpath@linetotoken {0.66667pt}{0pt}
  \pgfsyssoftpath@linetotoken {1pt}{0pt}
}
\tl_gset:cn {g__tilings_side_polykite_F_tl}
{
  \pgfsyssoftpath@movetotoken {0pt}{-2.00000070292pt}
  \pgfsyssoftpath@linetotoken {0.74999982427pt}{-1.566987221617321pt}
  \pgfsyssoftpath@linetotoken {1pt}{-2.00000070292pt}
}
\tl_gset:cn {g__tilings_side_polykite_f_tl}
{
  \pgfsyssoftpath@movetotoken {0pt}{2pt}
  \pgfsyssoftpath@linetotoken {0.25pt}{1.56699pt}
  \pgfsyssoftpath@linetotoken {1pt}{2pt}
}

\clist_map_inline:nn {a,A,b,B,f,F}
{
  \tl_gclear_new:c {g__tilings_side_backup_#1_tl}
  \tl_gset_eq:cc {g__tilings_side_backup_#1_tl} {g__tilings_side_#1_tl}
  \tl_gclear_new:c {g__tilings_side_#1_tl}
  \tl_gset_eq:cc {g__tilings_side_#1_tl}{g__tilings_side_polykite_#1_tl}
}

\BakeTile{subcluster~ H}
\BakeTile{subcluster~ T}
\BakeTile{subcluster~ P}
\BakeTile{subcluster~ F}

\clist_map_inline:nn {a,A,b,B,f,F}
{
  \tl_gset_eq:cc {g__tilings_side_#1_tl} {g__tilings_side_backup_#1_tl}
}
\cs_new_protected_nopar:Npn \__tilings_place_cluster_tile:nn #1#2
{
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \pgftransformscale{\fp_use:N \l__tilings_tmpa_fp}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \UseTile[
    every~ tile/.try,
    every~ #1~#2/.try,
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try/.expand~ once=\l__tilings_tmpc_tl
  ]{#1~ #2}
  \group_end:
}
\cs_generate_variant:Nn \__tilings_place_cluster_tile:nn {Vn}
\prop_new:N \g__tilings_supercluster_lms_rule_prop
\prop_gput:Nnn \g__tilings_supercluster_lms_rule_prop {T}
{
  [s H]
}
\prop_gput:Nnn \g__tilings_supercluster_lms_rule_prop {H}
{
  [s {r{-60}} T]
  [s {x{\fp_to_decimal:n{1}}} {y{\fp_to_decimal:n{(1+2*\c__tilings_phi_fp)}}} H]
  [s
    {x{\fp_to_decimal:n{-2-3*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-\c__tilings_phi_fp}}}
    H]
  [s
    {x{\fp_to_decimal:n{1+3*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-1-\c__tilings_phi_fp}}}
    {r{-120}}
    H]
  [s
    {x{\fp_to_decimal:n{-1.5-3.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{2.5*\c__tilings_phi_fp+1.5}}}
    {r{-120}}
    P]
  [s
    {x{\fp_to_decimal:n{-1.5-2*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-1.5-3*\c__tilings_phi_fp}}}
    {r{180}}
    P]
  [s
    {x{\fp_to_decimal:n{3+5.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{.5*\c__tilings_phi_fp}}}
    {r{120}}
    P]
  [s
    {x{\fp_to_decimal:n{-4.5-6.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{.5-.5*\c__tilings_phi_fp}}}
    {r{-120}}
    F]
  [s
    {x{\fp_to_decimal:n{1.5+4*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-2.5-3*\c__tilings_phi_fp}}}
    F]
  [s
    {x{\fp_to_decimal:n{3+2.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{2+3.5*\c__tilings_phi_fp}}}
    {r{120}}
    F]
}
\prop_gput:Nnn \g__tilings_supercluster_lms_rule_prop {P}
{
  [s {r{60}} P]
  [s
    {x{\fp_to_decimal:n{2.5+3.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-.5-.5*\c__tilings_phi_fp}}}
    {r{-120}}
    H]
  [s
    {x{\fp_to_decimal:n{-2.5-3.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{.5+.5*\c__tilings_phi_fp}}}
    {r{180}}
    H]
  [s
    {x{\fp_to_decimal:n{4.5+6*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{.5+\c__tilings_phi_fp}}}
    {r{120}}
    F]
  [s
    {x{\fp_to_decimal:n{-4.5-6*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-.5-\c__tilings_phi_fp}}}
    {r{-60}}
    F]
}
\prop_gput:Nnn \g__tilings_supercluster_lms_rule_prop {F}
{
  [s {r{60}} P]
  [s
    {x{\fp_to_decimal:n{2.5+3.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-.5-.5*\c__tilings_phi_fp}}}
    {r{-120}}
    H]
  [s
    {x{\fp_to_decimal:n{-2.5-3.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{.5+.5*\c__tilings_phi_fp}}}
    {r{180}}
    H]
  [s
    {x{\fp_to_decimal:n{4.5+6*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{.5+\c__tilings_phi_fp}}}
    {r{120}}
    F]
  [s
    {x{\fp_to_decimal:n{-4.5-6*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-.5-\c__tilings_phi_fp}}}
    {r{-60}}
    F]
  [s
    {x{\fp_to_decimal:n{3+4.5*\c__tilings_phi_fp}}}
    {y{\fp_to_decimal:n{-2-2.5*\c__tilings_phi_fp}}}
    F]
}
\prop_gput:Nnn \g__tilings_drawables_lms_prop {supercluster} {HTPF}
\fp_const:Nn \c__tilings_phi_fp {(1 + sqrt(5))/2}
\prop_new:N \g__tilings_supercluster_lms_action_prop

\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {r}
{
  \pgftransformrotate{\l__tilings_parameters_lms_tl}
}
\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {x}
{
  \pgftransformxshift{
    \fp_to_dim:n
    {.5 * (\l__tilings_parameters_lms_tl) * \l__tilings_step_dim}
  }
}
\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {y}
{
  \pgftransformyshift{
    \fp_to_dim:n
    {.5 * sqrt(3) * (\l__tilings_parameters_lms_tl) * \l__tilings_step_dim}
  }
}

\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {s}
{
  \fp_set:Nn \l__tilings_tmpa_fp {
    \l__tilings_step_dim
    /
    \c__tilings_phi_fp
    /
    \c__tilings_phi_fp
  }
  \dim_set:Nn \l__tilings_step_dim {\fp_to_dim:N \l__tilings_tmpa_fp}
}
\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {H}
{
  \__tilings_place_cluster_tile:nn {super~ cluster}{H}
}
\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {T}
{
  \__tilings_place_cluster_tile:nn {super~ cluster}{T}
}
\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {P}
{
  \__tilings_place_cluster_tile:nn {super~ cluster}{P}
}
\prop_gput:Nnn \g__tilings_supercluster_lms_action_prop {F}
{
  \__tilings_place_cluster_tile:nn {super~ cluster}{F}
}
\cs_new_protected_nopar:Npn \__tilings_place_cluster_tile_as_pic:nnnnnn #1#2#3#4#5#6
{
  \group_begin:
  \int_gincr:N \g__tilings_tile_int
  \fp_set:Nn \l__tilings_tmpa_fp {\l__tilings_step_dim/(1cm)}
  \tl_set:Nx \l__tilings_tmpc_tl
  {
    {\int_use:N  \g__tilings_tile_int}
    {\int_use:N \g__tilings_tiles_int}
  }
  \tl_clear:N \l__tilings_tmpa_tl
  \tl_put_right:Nn \l__tilings_tmpa_tl
  {
    \pic[
      every~ tile/.try,
      every~ #1~#2/.try,
    }
    \tl_put_right:Nx \l__tilings_tmpa_tl
    {
    tile~ \int_use:N \g__tilings_tile_int/.try,
    tile/.try=\l__tilings_tmpc_tl,
    scale=\fp_use:N \l__tilings_tmpa_fp,
    }
    \tl_put_right:Nn \l__tilings_tmpa_tl
    {
      name=#3,
    }
    \tl_if_empty:nTF {#4}
    {
      \tl_put_right:Nn \l__tilings_tmpa_tl
      {
        first~ tile/.try,
      }
    }
    {
      \tl_put_right:Nn \l__tilings_tmpa_tl
      {
        align~ with=#4~along~#5
      }
      \tl_if_single:nF {#6}
      {
        \tl_put_right:Nx \l__tilings_tmpa_tl
        {
          \c_space_tl using~\tl_tail:n {#6}
        }
      }
      \tl_put_right:Nn \l__tilings_tmpa_tl {,}
    }
    \tl_put_right:Nn \l__tilings_tmpa_tl
    {
      #1~ #2
    ];
  }
  \tl_use:N \l__tilings_tmpa_tl
  \group_end:
}
\cs_generate_variant:Nn \__tilings_place_cluster_tile_as_pic:nnnnnn {
  Vnnnnn, VnVnnn, VnVVnn
}
\tikzset{
  cluster~ type/.initial=super~ cluster,
  first~ file/.style={transform~ shape}
}
\prop_new:N \g__tilings_cluster_lms_rule_prop
\cs_new_nopar:Npn \__tilings_tile_label:
{
  \tl_item:Nn \l__tilings_parameters_lms_tl {1}
}
\cs_new_nopar:Npn \__tilings_adjoint_label:
{
  \tl_item:Nn \l__tilings_parameters_lms_tl {2}
}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {T}
{
  [s {H{\__tilings_tile_label:0}{}}]
}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {H}
{
  [s {r{-60}} {T{\__tilings_tile_label:0}{}}]
  [{ {HTa{A1}} {\__tilings_tile_label:1} {\__tilings_tile_label:0} }]
  [{ {HTa{A2}} {\__tilings_tile_label:2} {\__tilings_tile_label:0} }]
  [{ {HT{B1}b} {\__tilings_tile_label:3} {\__tilings_tile_label:0} }]
  [{ {PHb{B2}} {\__tilings_tile_label:4} {\__tilings_tile_label:1} }]
  [{ {PHb{B2}} {\__tilings_tile_label:5} {\__tilings_tile_label:2} }]
  [{ {PHAa} {\__tilings_tile_label:6} {\__tilings_tile_label:3} }]
  [{ {FHb{B1}} {\__tilings_tile_label:7} {\__tilings_tile_label:1} }]
  [{ {FHb{B1}} {\__tilings_tile_label:8} {\__tilings_tile_label:2} }]
  [{ {FHb{B2}} {\__tilings_tile_label:9} {\__tilings_tile_label:3} }]
}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {P}
{
  [s {r{60}} {P{\__tilings_tile_label:0}{}}]
  [{ {HPaA} {\__tilings_tile_label:1} {\__tilings_tile_label:0} }]
  [{ {HP{B2}b} {\__tilings_tile_label:2} {\__tilings_tile_label:0} }]
  [{ {FHb{B2}} {\__tilings_tile_label:3} {\__tilings_tile_label:1} }]
  [{ {FHb{B1}} {\__tilings_tile_label:4} {\__tilings_tile_label:2} }]
}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {F}
{
  [s {r{60}} {P{\__tilings_tile_label:0}{}}]
  [{ {HPaA} {\__tilings_tile_label:1} {\__tilings_tile_label:0} }]
  [{ {HP{B2}b} {\__tilings_tile_label:2} {\__tilings_tile_label:0} }]
  [{ {FHb{B2}} {\__tilings_tile_label:3} {\__tilings_tile_label:1} }]
  [{ {FHb{B1}} {\__tilings_tile_label:4} {\__tilings_tile_label:2} }]
  [{ {FHb{B1}} {\__tilings_tile_label:5} {\__tilings_tile_label:1} }]
}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {TH{A1}a} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {TH{A2}a} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {THb{B1}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {THb{B2}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HTa{A1}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HTa{A2}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HT{B1}b} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HT{B2}b} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HPaA} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HP{B1}b} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HP{B2}b} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HF{B1}b} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {HF{B2}b} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {PHAa} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {PHb{B1}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {PHb{B2}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {PF{11}{11}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {PF{12}{11}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {PF{11}{12}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {PF{12}{12}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FHb{B1}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FHb{B2}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FP{11}{11}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FP{12}{11}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FP{11}{12}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FP{12}{12}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FFfF} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FFFf} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FF{11}{11}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FF{12}{11}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FF{11}{12}} {}
\prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {FF{12}{12}} {}
\cs_new_nopar:cpn {__tilings_T{A1}_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {T#1{A1}#2}
  {
    [{ {H#3{B1}#4} {\__tilings_tile_label:0} {\__tilings_adjoint_label:#5} }]
  }
}
\cs_new_nopar:cpn {__tilings_T{A2}_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {T#1{A2}#2}
  {
    [{ {H#3{B2}#4} {\__tilings_tile_label:0} {\__tilings_adjoint_label:#5} }]
  }
}
\cs_new_nopar:cpn {__tilings_Tb_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {T#1b#2}
  {
    [{ {H#3a#4} {\__tilings_tile_label:0} {\__tilings_adjoint_label:#5} }]
  }
}

\cs_new_nopar:cpn {__tilings_H{B1}_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {H#1{B1}#2}
  {
    [{ {P#3A#4} {\__tilings_tile_label:4} {\__tilings_adjoint_label:#5} }]

    [{ {HP{B2}b} {\__tilings_tile_label:1} {\__tilings_tile_label:4} }]
    [{ {TH{A1}a} {\__tilings_tile_label:0} {\__tilings_tile_label:1} }]

    [{ {HTa{A2}} {\__tilings_tile_label:2} {\__tilings_tile_label:0} }]
    [{ {PHb{B2}} {\__tilings_tile_label:5} {\__tilings_tile_label:2} }]

    [{ {HT{B1}b} {\__tilings_tile_label:3} {\__tilings_tile_label:0} }]
    [{ {PHAa} {\__tilings_tile_label:6} {\__tilings_tile_label:3} }]

    [{ {FHb{B1}} {\__tilings_tile_label:7} {\__tilings_tile_label:1} }]
    [{ {FHb{B1}} {\__tilings_tile_label:8} {\__tilings_tile_label:2} }]
    [{ {FHb{B2}} {\__tilings_tile_label:9} {\__tilings_tile_label:3} }]
  }
}

\cs_new_nopar:cpn {__tilings_H{B2}_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {H#1{B2}#2}
  {
    [{ {P#3A#4} {\__tilings_tile_label:5} {\__tilings_adjoint_label:#5} }]

    [{ {HP{B2}b} {\__tilings_tile_label:2} {\__tilings_tile_label:5} }]
    [{ {TH{A2}a} {\__tilings_tile_label:0} {\__tilings_tile_label:2} }]

    [{ {HTa{A1}} {\__tilings_tile_label:1} {\__tilings_tile_label:0} }]
    [{ {PHb{B2}} {\__tilings_tile_label:4} {\__tilings_tile_label:1} }]

    [{ {HT{B1}b} {\__tilings_tile_label:3} {\__tilings_tile_label:0} }]
    [{ {PHAa} {\__tilings_tile_label:6} {\__tilings_tile_label:3} }]

    [{ {FHb{B1}} {\__tilings_tile_label:7} {\__tilings_tile_label:1} }]
    [{ {FHb{B1}} {\__tilings_tile_label:8} {\__tilings_tile_label:2} }]
    [{ {FHb{B2}} {\__tilings_tile_label:9} {\__tilings_tile_label:3} }]
  }
}

\cs_new_nopar:cpn {__tilings_Ha_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {H#1a#2}
  {
    [{ {P#3b#4} {\__tilings_tile_label:6} {\__tilings_adjoint_label:#5} }]

    [{ {HPaA} {\__tilings_tile_label:3} {\__tilings_tile_label:6} }]
    [{ {THb{B1}} {\__tilings_tile_label:0} {\__tilings_tile_label:3} }]

    [{ {HTa{A1}} {\__tilings_tile_label:1} {\__tilings_tile_label:0} }]
    [{ {PHb{B2}} {\__tilings_tile_label:4} {\__tilings_tile_label:1} }]

    [{ {HTa{A2}} {\__tilings_tile_label:2} {\__tilings_tile_label:0} }]
    [{ {PHb{B2}} {\__tilings_tile_label:5} {\__tilings_tile_label:2} }]

    [{ {FHb{B1}} {\__tilings_tile_label:7} {\__tilings_tile_label:1} }]
    [{ {FHb{B1}} {\__tilings_tile_label:8} {\__tilings_tile_label:2} }]
    [{ {FHb{B2}} {\__tilings_tile_label:9} {\__tilings_tile_label:3} }]
  }
}

\cs_new_nopar:cpn {__tilings_PA_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {P#1A#2}
  {
    [{ {H#3{B1}#4} {\__tilings_tile_label:1} {\__tilings_adjoint_label:#5} }]
    [{ {PHAa} {\__tilings_tile_label:0} {\__tilings_tile_label:1} }]
    [{ {HP{B2}b} {\__tilings_tile_label:2} {\__tilings_tile_label:0} }]

    [{ {FHb{B2}} {\__tilings_tile_label:3} {\__tilings_tile_label:1} }]
    [{ {FHb{B1}} {\__tilings_tile_label:4} {\__tilings_tile_label:2} }]
  }
}

\cs_new_nopar:cpn {__tilings_Pb_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {P#1b#2}
  {
    [{ {H#3a#4} {\__tilings_tile_label:2} {\__tilings_adjoint_label:#5} }]
    [{ {PHb{B2}} {\__tilings_tile_label:0}{\__tilings_tile_label:2} }]
    [{ {HPaA} {\__tilings_tile_label:1} {\__tilings_tile_label:0} }]

    [{ {FHb{B2}} {\__tilings_tile_label:3} {\__tilings_tile_label:1} }]
    [{ {FHb{B1}} {\__tilings_tile_label:4} {\__tilings_tile_label:2} }]
  }
}

\cs_new_nopar:cpn {__tilings_Fb_creator:nnnnn} #1#2#3#4#5
{
  \prop_gput:Nnn \g__tilings_cluster_lms_rule_prop {F#1b#2}
  {
    [{ {H#3a#4} {\__tilings_tile_label:2} {\__tilings_adjoint_label:#5} }]
    [{ {PHb{B2}} {\__tilings_tile_label:0}{\__tilings_tile_label:2} }]
    [{ {HPaA} {\__tilings_tile_label:1} {\__tilings_tile_label:0} }]

    [{ {FHb{B2}} {\__tilings_tile_label:3} {\__tilings_tile_label:1} }]
    [{ {FHb{B1}} {\__tilings_tile_label:4} {\__tilings_tile_label:2} }]
    [{ {FHb{B1}} {\__tilings_tile_label:5} {\__tilings_tile_label:1} }]
  }
}
\clist_map_inline:nn
{
  TH{{A1}}a HP{{{B1}}}b06,
  TH{{A2}}a HP{{{B2}}}b06,
  THb{{B1}} HPaA04,
  THb{{B2}} HPaA05,
  PHAa HP{{{B1}}}b16,
  PHb{{B1}} HPaA24,
  PHb{{B2}} HPaA25,
  FHb{{B1}} HPaA24,
  FHb{{B2}} HPaA25,
}
{
  \tl_clear:N \l__tilings_tmpa_tl
  \tl_put_right:Nn \l__tilings_tmpa_tl { \use:c }
  \tl_put_right:Nx \l__tilings_tmpa_tl
  {
    {__tilings_ \tl_item:nn {#1}{2}\tl_item:nn {#1}{4} _creator:nnnnn}
    {\tl_item:nn {#1}{1}}{\tl_item:nn{#1}{3}}
    \tl_item:nn {#1}{5}\tl_item:nn{#1}{7}
    \tl_item:nn {#1}{9}
  }
  \tl_use:N \l__tilings_tmpa_tl
  \tl_clear:N \l__tilings_tmpa_tl
  \tl_put_right:Nn \l__tilings_tmpa_tl { \use:c }
  \tl_put_right:Nx \l__tilings_tmpa_tl
  {
    {__tilings_ \tl_item:nn {#1}{1}\tl_item:nn {#1}{3} _creator:nnnnn}
    {\tl_item:nn {#1}{2}}{\tl_item:nn{#1}{4}}
    \tl_item:nn {#1}{6}\tl_item:nn{#1}{8}
    \tl_item:nn {#1}{10}
  }
  \tl_use:N \l__tilings_tmpa_tl
}

\prop_new:N \g__tilings_cluster_lms_action_prop
\prop_gput:Nnn \g__tilings_drawables_lms_prop {cluster} {HTPF}
\prop_gput:Nnn \g__tilings_cluster_lms_action_prop {r}
{
  \pgftransformrotate{\l__tilings_parameters_lms_tl}
}
\prop_gput:Nnn \g__tilings_cluster_lms_action_prop {x}
{
  \pgftransformxshift{
    \fp_to_dim:n
    {.5 * (\l__tilings_parameters_lms_tl) * \l__tilings_step_dim}
  }
}
\prop_gput:Nnn \g__tilings_cluster_lms_action_prop {y}
{
  \pgftransformyshift{
    \fp_to_dim:n
    {.5 * sqrt(3) * (\l__tilings_parameters_lms_tl) * \l__tilings_step_dim}
  }
}

\prop_gput:Nnn \g__tilings_cluster_lms_action_prop {s}
{
  \fp_set:Nn \l__tilings_tmpa_fp {
    \l__tilings_step_dim
    /
    \c__tilings_phi_fp
    /
    \c__tilings_phi_fp
  }
  \dim_set:Nn \l__tilings_step_dim {\fp_to_dim:N \l__tilings_tmpa_fp}
}
\clist_map_inline:nn {H,T,P,F}
{

  \prop_gput:Nnn \g__tilings_cluster_lms_action_prop {#1}
  {
    \__tilings_tikz_keys_get:Nn \l__tilings_tmpa_tl {cluster~type}
    \tl_set:Nx \l__tilings_tmpb_tl {\tl_item:Nn \l__tilings_parameters_lms_tl {1}}
    \__tilings_place_cluster_tile_as_pic:VnVnnn
    \l__tilings_tmpa_tl {#1} \l__tilings_tmpb_tl {}{}{}
  }
}
\cs_new_protected_nopar:Npn \__tilings_place_cluster_tile_as_pic_aux:nnnn #1#2#3#4
{
  \__tilings_tikz_keys_get:Nn \l__tilings_tmpa_tl {cluster~type}
  \tl_set:Nx \l__tilings_tmpb_tl {\__tilings_tile_label:}
  \tl_set:Nx \l__tilings_tmpc_tl {\__tilings_adjoint_label:}
  \__tilings_place_cluster_tile_as_pic:VnVVnn
  \l__tilings_tmpa_tl {#1} \l__tilings_tmpb_tl \l__tilings_tmpc_tl {#4}{#3}
}

\clist_map_inline:nn {
  TH{A1}a,
  TH{A2}a,
  THb{B1},
  THb{B2},
  HTa{A1},
  HTa{A2},
  HT{B1}b,
  HT{B2}b,
  HPaA,
  HP{B1}b,
  HP{B2}b,
  HF{B1}b,
  HF{B2}b,
  PHAa,
  PHb{B1},
  PHb{B2},
  PF{11}{11},
  PF{12}{11},
  PF{11}{12},
  PF{12}{12},
  FHb{B1},
  FHb{B2},
  FP{11}{11},
  FP{12}{11},
  FP{11}{12},
  FP{12}{12},
  FFfF,
  FFFf,
  FF{11}{11},
  FF{12}{11},
  FF{11}{12},
  FF{12}{12}
}
{
  \prop_gput:Nnn \g__tilings_cluster_lms_action_prop {#1}
  {
    \__tilings_place_cluster_tile_as_pic_aux:nnnn #1
  }
}

\ExplSyntaxOff
%% 
%% Copyright (C) 2014-2023 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  penrose_code.dtx
%%                                  penrose.tex
%% and the derived files            penrose.ins
%%                                  penrose_code.pdf
%%                                  penrose.pdf
%%                                  tikzlibrarytilings.code.tex
%%                                  tikzlibrarytilings.penrose.code.tex
%%                                  tikzlibrarytilings.polykite.code.tex
%%                                  tikzlibrarypenrose.code.tex
%%                                  README.txt
%% 
%%
%% End of file `tikzlibrarytilings.polykite.code.tex'.

